Secure System Virtualization: End-to-End Verification of Memory Isolation

Over the last years, security kernels have played a promising role in reshaping the landscape of platform security on today's ubiquitous embedded devices. Security kernels, such as separation kernels, enable constructing high-assurance mixed-criticality execution platforms. They reduce the software portion of the system's trusted computing base to a thin layer, which enforces isolation between low- and high-criticality components. The reduced trusted computing base minimizes the system attack surface and facilitates the use of formal methods to ensure functional correctness and security of the kernel. In this thesis, we explore various aspects of building a provably secure separation kernel using virtualization technology. In particular, we examine techniques related to the appropriate management of the memory subsystem. Once these techniques were implemented and functionally verified, they provide reliable a foundation for application scenarios that require strong guarantees of isolation and facilitate formal reasoning about the system's overall security.

==> cacheBleed/commands.tex <==
\newenvironment{defn}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{invariant}{Invariant}
\newtheorem{axiom}{Axiom}
\newtheorem{assumption}{Assumption}
\newcommand{\similar}[3]{\similarrel{#1}(#2,#3)}
\newcommand{\similarrel}[1]{sim_#1}
\newcommand{\armv}{ARMv7}
\newcommand{\MMU}{\mathit{mmu}}
\newcommand{\timeFun}{t}


\newcommand{\emptymsg}{\perp}
\newcommand{\ModeSet}{\mathcal{M}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\idx}{id}
\newcommand{\Exe}{\pi}
\newcommand{\Trace}{\omega}
\newcommand{\TraceSet}[2]{\mathit{tr}_{#1,#2}}
\newcommand{\TraceSetb}[1]{\mathit{tr}_{#1}}
\newcommand{\map}{\mathit{map}}
\newcommand{\project}{\mathit{prj}}
\newcommand{\ActiveGuestReal}[1]{\mathit{act}_#1}
\newcommand{\ActiveGuestIdeal}[1]{\mathit{act}_#1}
\newcommand{\Seq}{\pi}
\newcommand{\Pred}{\phi}
\newcommand{\Trans}[1]{\xrightarrow{}}
\newcommand{\PrivTrans}[1]{\overset{#1}{\rightsquigarrow}}
%\mathrel{\mathop{\rightsquigarrow}^{#1}}}
\newcommand{\ArmStateSpace}{\Sigma}
\newcommand{\RealStateSpace}{\mathcal{S}}
% USED for real states with no cache
\newcommand{\RealStateSpaceAbs}{\overline {\mathcal{S}}}
\newcommand{\IdealStateSpace}{\mathcal{Q}}
\newcommand{\HyperDataSpace}{\mathcal{H}}
%\newcommand{\ArmState}{\texttt{$\sigma$}}
\newcommand{\ArmState}{s}
\newcommand{\RealState}{s}
\newcommand{\IdealState}{q}
\newcommand{\IdealMachines}{\Gamma}
\newcommand{\IdealMachine}{\sigma}
% USED for TLS states with no cache
\newcommand{\IdealMachineAbs}{\bar \sigma}

\newcommand{\Req}{\mathit{req}}

\newcommand{\Memory}{\mathit{mem}}
\newcommand{\cache}{\mathit{cache}}
\newcommand{\mainMemory}{\mathit{mem}}
\newcommand{\gCompatible}[2]{{(#1,#2)\rm{\textit{-compatible}}}}
\newcommand{\Untouched}[3]{\mathit{unmodified}_#1(#2,#3)}
\newcommand{\PrivilegedConst}[3]{\mathit{priv\_const}_#1(#2,#3)}
\newcommand{\PrivilegedConstOP}{\mathit{priv\_const}}
\newcommand{\ActiveGuest}{ag}
\newcommand{\LTS}[4]{#1=\langle #2,#3,#4\rangle}
\newcommand{\gLTS}{\rm{GT}}
\newcommand{\SPSR}{\mathit{psr}}
\newcommand{\CPSR}{\mathit{cpsr}}
\newcommand{\ProofCase}[1]{
\vskip 10pt
\noindent Case \underline{#1:}
}
\newcommand{\ModeOp}{mode}
\newcommand{\Mode}[1]{\ModeOp(#1)}
\newcommand{\mode}[1]{\ModeOp(#1)}
\newcommand{\PROSPER}{PROSPER}
\newcommand{\caEq}[2]{#1 \equiv_{ca} #2 }
\newcommand{\impl}{\Rightarrow}
\newcommand{\fall}{$\forall$}
\newcommand{\conj}{$\wedge$}
\newcommand{\thereis}{$\exists$}
\newcommand{\mmueq}{\equiv_{mmu}}
\newcommand{\RelP}{\mathrel{\mathcal{P}}}


\newcommand{\GuestMemType}{0}
\newcommand{\SecMemType}{1}
\newcommand{\DataType}{\textit{data}}
\newcommand{\LTwoType}{\textit{L2}}
\newcommand{\LOneType}{\textit{L1}}

\newcommand{\UserMode}{\mathit{PL0}}
\newcommand{\KernelMode}{\mathit{PL1}}
\newcommand{\Sec}{S}
\newcommand{\coregs}{\mathit{coregs}}
\newtheorem{property}{Property}
\newcommand{\HypState}{h}
\newcommand{\secureObs}[1]{O_s(#1)}

\newcommand{\C}{\mathbb{C}}
\renewcommand{\L}{\mathbb{L}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\T}{\mathbb{T}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\VA}{\mathit{VA}}
\newcommand{\PA}{\mathit{PA}}
\newcommand{\ow}{\mathrm{otherwise}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}

\newcommand{\RegVar}{R}
\newcommand{\MemVar}{M}
\newcommand{\CoRegVar}{\mathit{CR}}
\newcommand{\CacheVar}{C}
\newcommand{\LogVar}{k}

\newcommand{\wordX}{\B^{8}}
\newcommand{\wordY}{\B^{32}}

\newcommand{\RegionGuest}{\mathbf{G}}
\newcommand{\RegionGuestCache}{\mathbf{C}}
\newcommand{\RegionGuestNonCache}{\mathbf{\overline C}}
\newcommand{\RegionHyper}{\mathbf{H}}

\newcommand{\TlsStateVar}{\IdealState}
\newcommand{\ArmMachineVar}{\ArmState}
\newcommand{\BisimR}{\mathrel{\mathcal{R}}}
\newcommand{\BisimAbsR}{\mathrel{\mathcal{R}^a}}
\newcommand{\AbsR}{\ \mathcal{A}\ }

% USED for real states with no cache
\newcommand{\ArmMachineAbsVar}{\bar \ArmState}

% Atomic kernel function, like DMMU, in the ISA TLS
\newcommand{\TlsFunctionAbs}{\mathbf{\bar F}}
% Atomic kernel function, like DMMU, in the real TLS
\newcommand{\TlsFunction}{\mathbf{F}}

\newcommand{\op}[1]{\ #1 \ }

\newcommand{\CacheFromPA}{D}
\newcommand{\obs}{O}

\newcommand{\integral}{sec}


% \newcommand{\revision}[4]{
%   {\color{green}{[#1:#2]}}
%   {\color{red}{#3}}
%   {\color{blue}{#4}}
% }
% \newcommand{\revision}[4]{
%   \marginpar{\color{green}{[#1:#2]}}
%   {\color{blue}{#4}}
% }
\newcommand{\revision}[4]{#4}

\newcommand{\rev}[3]{R#1:#2-#3}
\newcommand{\hamedR}[3]{\revision{Hamed}{#1}{#2}{#3}}
\newcommand{\guancioR}[3]{\revision{Roberto}{#1}{#2}{#3}}
\newcommand{\mfdR}[3]{\revision{Mads}{#1}{#2}{#3}}
\newcommand{\cbauR}[3]{\revision{Christoph}{#1}{#2}{#3}}


==> cacheBleed/platform.tex <==
\section{Virtualization Platform}\label{REAL}
As basis for the study we use a hypervisor~\cite{Nemati2015} running on an
\armv~Cortex-A8 processor~\cite{ARMv7}. However, the problems we
identify, and the solutions we propose, are general and apply to other 
SW and HW platforms as well, including, at least in part, those with hardware
virtualization support. 

A peculiarity of the hypervisor (and others \cite{XEN}) that makes it 
particularly relevant for our purpose is the direct paging 
mechanism, which allows guests to set up the page tables that will be 
used for translation later, i.e., there is no hypervisor-controlled second 
stage translation. 

The \armv~machine state is modelled as a record $\ArmState = \tuple{
  \RegVar,  \MemVar, \CacheVar, \CoRegVar} \in \RealStateSpace$ 
containing the registers, memory, data-cache, and coprocessors of the machine.
The processor executes in $\ModeOp(\ArmState) \in
\{\UserMode,\KernelMode\}$; where $\UserMode$ is the non-privileged
mode and  $\KernelMode$ is the privileged one. Memory and cache are modeled as
presented in Section~\ref{sec:generic:cache}. We do not go into the
details of instantiating the cache for the Cortex-A8 processor here. These details are
irrelevant to the verification methodology. For simplicity, we limit the 
discussion to the L1 caches. Moreover, we assume that
caches are updated deterministically, i.e., we do not
account  for effects on the cache due to hardware functionality that is
invisible to the programmer, e.g., speculative execution. 
%See Section~\ref{cache proof} for a deeper discussion of the topic. 

Component $\CoRegVar$ represents coprocessor registers controlling the
Memory Management Unit (MMU). These registers determine among other things
whether MMU and caches are enabled and they hold the base address of
the current page table. Entries of the page table encode a
virtual-to-physical mapping for a memory page as well as access
permissions. 

Function $mmu(\ArmState, \mathit{PL}, va, req)$, defines the address
translation, mapping virtual addresses $va$ and requests $req \in
\{rd, wt, ex\}$ (representing read, write, execute) to either a pair
$(pa,c) \in (\mathit{PA} \times \B)$ or $\bot$. 
If the result is undefined, e.g., due to insufficient
privileges for a memory access, a page fault occurs. Otherwise the
Boolean component of the pair denotes whether the address is cacheable
or not. On \armv~ the address translation depends on the page
tables stored in the memory. Moreover, on Cortex-A8 the MMU
consults the data cache before accessing the main memory whenever a
page table descriptor must be fetched.

The behavior of the processor is defined by transition relation
$\rightarrow \subseteq \RealStateSpace \times \RealStateSpace$.
Non-privileged transitions start from and end in non-privileged mode states.
All the other transitions  involve at least one state in the privileged mode.
Only exceptions, e.g., page faults, can bring the system from
$\UserMode$ to $\KernelMode$. A special case of this are software
interrupts (SWI) which can be triggered using system call
instructions.


The architecure is paravirtualized by the hypervisor for
several operating systems (guests). In this paper
we limit ourselves to treating two separate guests. Only the
hypervisor is executing in privileged mode,
while the guests are executed in non-privileged mode and need to
invoke hypervisor functionality to alter the critical resources of the
system.  %% To implement the virtualization
%% the hypervisor needs to distinguish two virtual CPU modes: virtual
%% user and kernel mode, each with their own execution context, however
%% for our cache analysis the virtual guest CPU mode is irrelevant.
At all times, only one guest is running while the other one is
inactive. A cooperative scheduling policy allows to reschedule
inactive guests whenever the active guest explicitly releases the usage of the
CPU.

The machine memory is partitioned into three separate regions: region $\RegionGuest_g$ 
for the guest $g \in \{1,2\}$, and a hypervisor memory region
$\RegionHyper$. The hypervisor guarantees non-interference between
these memory segments by monitoring the configuration of the MMU.
The MMU is a critical resource since it provides memory
protection and any misconfiguration (via manipulation of page tables) allows malicious
applications to gain illicit access.
The hypervisor virtualizes the MMU using direct-paging, enabling 
a guest to manage its own memory space with assistance of the hypervisor. 
This approach has been
previously introduced by Xen~\cite{XEN}. Direct paging allows the
guest to allocate the page tables inside its own memory and to
directly manipulate them while the tables are not in active use by the
MMU. The hypervisor provides a number of system calls (whose set is
called DMMU) that supports
the allocation, deallocation, linking, and activation of guest page
tables. These calls need to validate that the proposed setup of the
MMU does not introduce any illicit access grant, by
reading the page tables located in guest memory. 





%% These reads open the
%% door for cache-based side channel attacks on the integrity of
%% isolation guaranteed by the hypervisor.
  


==> cacheBleed/proof.tex <==
We split the task to  prove the theorem (\ref{eq:TopLevelGoal}) in two parts: i) proving that partition observations are the same in the real and the ideal systems, ii) and then 
ensuring that execution of the kernel handlers terminates, and user states in the ideal and the real worlds remain  compatible when the control returns back to the partitions.

\paragraph{$(g,m)$-Compatible States}
In order to ensure that the partition observations are the same in the real and the ideal systems, 
We briefly define the conditions for the user mode states (i.e. when all machines are in the user mode) and the switched mode states 
(i.e. the inactive machine of ideal machine is in the user mode but the real system and the active machine of ideal system have recently switched to the privileged mode). 

Say that two states $\RealState$ and $\IdealState$ are $\gCompatible{g}{m}$ if
(i) $\RealState$ and $\IdealState$ are in the mode $m$,
(ii) $g$ is the last active partition in $\RealState$ and $\IdealState$,
i.e. the status of the domain $g$, held by coprocessor register $c_3$ is client in $\RealState$,
and the $\idx$ field of the ideal state is $g$,
(iii) the partitions have the same observations in $\RealState$ and $\IdealState$, $O_{g'}(\RealState)=O_{g'}(\IdealState)$ for $g' \in \{1,2\}$,
(iv) the values of data-structures in the logical component of state $\IdealState$ agree with the values of  corresponding data structures in the kernel
of state $\RealState$, 
(v) the MMU and coprocessors are configured correctly in all three machines,
(vi) a set of invariants are held by the kernel data-structure in $\RealState$.

\paragraph{User/Handler Lemmas}
The relation of (\textit{g,m})-compatibility is our candidate unwinding relation, i.e. it is in some suitable sense which we go on to make precise preserved under computation.
This involves showing the following two key properties:
\begin{itemize}
\item User Lemma: Each user mode transition in the real system is matched (in the sense of (\textit{g,m})-compatibility) by a corresponding user mode transition in 
the ideal system without interfering with the resources that are not intended to be accessible by the partition, and vice versa.
\item Handler Lemma: Each complete handler execution in the real system is matched (as (\textit{g,m})-compatibility) by a corresponding execution of a 
kernel functionality in the ideal model, and vice versa.
\end{itemize}
% Similar to the $\mathit{unmodified}_g$ predicate for the real system above, $\Untouched{g}{\IdealState}{\IdealState'}$ holds if 
% the logical component, the inactive machine, and the non-accessible resources of the active machine are unmodified by an ideal transition from $\IdealState$ to $\IdealState'$ when $g$ is active in $\IdealState$. The User Lemma then follows from the first and second ARM Lemmas as follows:
Further we define $\Untouched{g}{\RealState}{\RealState'}$ as a relation stating that the non-accessible resources for a state $\RealState$ in user mode, including the coprocessor registers and the memory regions not allocated to the active partition $g$,
are not modified in a transition from $\RealState$ to another user mode state ${\RealState'}$.

We start with user lemma and then elaborate more on handlers lemma in the section \ref{}.
Formally we define user lemma as following:

\begin{lemma}[User]\label{lem:user.lemma}
%\textbf{User Lemma}
For all $\gCompatible{g}{PL0}$ states $\RealState$ and $\IdealState$,
if $\IdealState \to \IdealState'$ then 
there exist $\RealState'$ and $m$ such that
\begin{itemize}
\item[(i)] $\RealState \to \RealState'$, 
\item[(ii)] the states $\RealState'$ and $\IdealState'$ are
$\gCompatible{g}{m}$,
%\item[(iii)] $\secureObs{\RealState} = \secureObs{\RealState'}$, and (iv) $\secureObs{\IdealState} = \secureObs{\IdealState'}$.
\item[(iii)] $\Untouched{g}{\RealState}{\RealState'}$, and (iv) $\Untouched{g}{\IdealState}{\IdealState'}$.
\end{itemize}
Vice versa, if $\RealState \to \RealState'$ then $\IdealState'$ and $m$ exists such that $\IdealState \to \IdealState'$ and the above properties (ii) and (iii) hold.
\end{lemma}

This lemma follows from two ARM user lemmas: 
\begin{enumerate}
 \item 
 \begin{lemma}{(informal definition):}
 \label{lem:first.ARM.lemma} 
  The first lemma is a general noninterference lemma stating that if an ARM machine executes in user mode in a memory protected
  configuration, the behavior of the active partition is influenced only by those resources allowed to do so.
 \end{lemma}
% The predicate $\similar{g}{\RealState_1}{\RealState_2}$ indicates
%  that the status of the domain $g$ held by coprocessor register $c_3$ is client
%  in the user mode states $\RealState_1$ and $\RealState_2$, and 
%  they have the same user registers, MMU configurations and 
%  the memory and cache lines allocated to the domain $g$.
%  
% \begin{lemma}
% \label{lem:first.ARM.lemma}
% If $\similar{g}{\RealState_1}{\RealState_2}$ and
% $\RealState_1 \to \RealState_1'$,
% there exists $\RealState_2'$ s.t. $\RealState_2 \to \RealState_2'$ 
% and $\similar{g}{\RealState'_1}{\RealState'_2}$,
% and vice versa.
% \end{lemma}

 \item 
 \begin{lemma}{(informal definition):}
 \label{lem:second.ARM.lemma} 
  The second lemma establishes $\Untouched{g}{\RealState}{\RealState'}$ relation.  
 \end{lemma}


% \begin{lemma}
% \label{lem:second.ARM.lemma}
% If $\RealState \to \RealState'$ and
% $\ActiveGuestReal{g}(\RealState)$ then
% $\Untouched{g}{\RealState}{\RealState'}$.
% \end{lemma}

\end{enumerate}

The next section gives a more precise definition of these two lemmas and shows how they can be proved using guarantees provided  by the CPU.


\subsection{ARM user lemmas}\label{sec:armLemmas}

Intuitively, guaranteeing spatial isolation means confining the guest
to manage a part of the physical memory available for the guest uses. 
In our setting, this part is determined statically and identified by the predicate
$G_{g.m}(pa)$, which holds if the physical address $pa$ is part of the
physical memory assigned to the guest partition.
Clearly, no security property can be guaranteed if the system
starts from a non-consistent state; for example the guest can not be allowed to change the MMU behavior by directly writing the page tables.
For this reason we introduce a system invariant $I(\tuple{\ArmState,
  h})$ that is used to constrain the set of consistent initial states
of the TLS. We use $\IdealStateSpace_I$ to represent the set of all possible TLS
states that satisfy the invariant. We thus need to show:
%
\begin{theorem}\label{lem:invariant}
  Let $\tuple{s,h} \in \IdealStateSpace_I$ and $i\in\{0,1\}$.
  If 
  $\tuple{s,h} \to_i \tuple{s',h'}$
  then
  $I(\tuple{s',h'})$.
\end{theorem}
%
Next sub-section elaborates the definition of the invariant and
 summarizes the proof of the Theorem.
 
We say that two states are \textit{MMU-equivalent} if for any virtual
address $va$ the MMU yields the same translation and the same access
permissions. Formally,  $\ArmState \equiv_{mmu} \ArmState'$ if and
only if 
$$\ mmu(\ArmState, PL, va, req) = mmu(\ArmState', PL, va, req)$$
for any $va$, $PL$, $req$. Complete mediation (MMU-integrity) is demonstrated by showing
that the guest is not able to directly change the content of the page tables and affect the address translation mechanism.
\begin{theorem}\label{lem:mmu-integrity}
  Let $\tuple{s,h} \in \IdealStateSpace_I$.
  If $\tuple{s,h} \to_0 \tuple{s',h'}$
  then
  $s \equiv_{mmu} s'$.
\end{theorem}

We use the approach of~\cite{Heitmeyer:2008:AFM:1340674.1340715} to
analyze the hypervisor data separation properties.
The observations of the guest in a state $\tuple{s,h}$ is represented by the
structure $O_g(\tuple{s,h}) = \tuple{ \mathit{\mainMemory}_g, \mathit{cache}_g, \mathit{uregs}, \mathit{coregs}}$, which is similar to the observation of the guest in state $s$ or $O_g(s)$.
The coprocessor registers are visible to the guest since they directly affect guest behaviour, and do not contain any
information the guest should not be allowed to see. 
Evidently, however, all writes to the coprocessor registers
must be mediated by the hypervisor.

The remaining part of the state (i.e. resources that are subject of $unmodified$ relation) constitute the secure observations $O_s(\tuple{s,h})$
of the state, which guest transitions are not supposed to affect.

The lemma \ref{lem:first.ARM.lemma} is called \emph{non-infiltration} and that is a non-interference property
guaranteeing that guest instructions and hypercalls
executed on behalf of the guest do not depend on any information stored in
resources not accessible by the guest.
\begin{theorem}\label{lem:No-Infiltration}
  Let
  $\tuple{s_1,h_1} ,\tuple{s_2,h_2}  \in \IdealStateSpace_I$, $i \in\{0,1\}$,
  and assume  that 
  $O_{g}(\tuple{s_1,h_1}) = O_{g}(\tuple{s_2,h_2})$.
  If $\tuple{s_1,h_1} \to_i \tuple{s'_1,h'_1}$ and
  $\tuple{s_2,h_2} \to_i \tuple{s'_2,h'_2}$
  then
  $O_{g}(\tuple{s'_1,h'_1}) = O_{g}(\tuple{s'_2,h'_2})$.
\end{theorem}


Similarly we call the lemma \ref{lem:second.ARM.lemma} \emph{non-exfiltration} that is  property guaranteeing  that 
a transition executed by the guest 
does not modify the secure resources:

\begin{theorem}\label{lem:No-Exfiltration}
  Let $\tuple{s,h} \in \IdealStateSpace_I$.
  If $\tuple{s,h} \to_0 \tuple{s',h'}$ 
  then
  $O_s(\tuple{s,h}) = O_s(\tuple{s',h'})$.
\end{theorem}


\input{user-mode_lemma-proof}

==> jcs/macros.tex <==
\newenvironment{defn}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{definition}{Definition}

\newcommand{\SCTLR}{SCTLR}
\newcommand{\TTBRzero}{TTBR0}
\newcommand{\DACR}{DACR}
\newcommand{\Mem}{\texttt{mem}}
\newcommand{\PL}{\texttt{pl}}
\newcommand{\priv}{\mathit{mode}}
\newcommand{\regs}{\mathit{regs}}
\newcommand{\psrs}{\mathit{psrs}}
\newcommand{\coregs}{\mathit{coregs}}
\newcommand{\mem}{\mathit{mem}}
\newcommand{\HypState}{h}
\newcommand{\pgtype}{\mathit{pgtype}}
\newcommand{\pgrefs}{\mathit{pgrefs}}
\newcommand{\mode}{\mathit{mode}}
\newcommand{\refs}{\mathit{refs}}
\newcommand{\Data}{\mathit{D}}
\newcommand{\sound}{\mathit{sound}}
\newcommand{\type}{\mathit{pgtype}}
\newcommand{\countt}{\mathit{count}}
\newcommand{\block}{\mathit{block}}
\newcommand{\fnsize}{\footnotesize \mathit{size}}
\newcommand{\fnref}{\footnotesize \mathit{ref}}

\newcommand{\ineq}{$\neq$}
\newcommand{\negat}{$\neg$}
\newcommand{\fall}{$\forall$}
\newcommand{\impl}{$\Rightarrow$}
\newcommand{\sigmas}{$\sigma$}
\newcommand{\botm}{$\bot$}
\newcommand{\wrt}{\ensuremath{\texttt{write}_{32}}}
\newcommand{\rd}{\ensuremath{\texttt{read}_{32}}}
\newcommand{\mmu}[1]{\ensuremath{\texttt{mmu}_{#1}}}
\newcommand{\mathunderline}[2]{\ensuremath{\texttt{#1}_{#2}}}
\newcommand{\equivs}[1]{$\equiv_{#1}$}
\newcommand{\ActiveGuestReal}[1]{\mathit{act}_#1}
\newcommand{\ActiveGuestIdeal}[1]{\mathit{act}_#1}
\newcommand{\Trace}{\omega}
\newcommand{\project}{\mathit{prj}}
\newcommand{\map}{\mathit{map}}
\newcommand{\TraceSet}[2]{\mathit{tr}_{#1,#2}}
\newcommand{\TraceSetb}[1]{\mathit{tr}_{#1}}

\newcommand{\armv}{ARMv7}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\RealStateSpace}{\Sigma}
\newcommand{\ArmState}{\sigma}
\newcommand{\UserMode}{\mathit{PL0}}
\newcommand{\KernelMode}{\mathit{PL1}}
\newcommand{\IdealStateSpace}{\mathcal{Q}}
\newcommand{\Exe}{\pi}
\newcommand{\Sec}{S}
\newcommand{\PLm}{\mathit{pl}}
\newcommand{\req}{\mathit{req}}
\newcommand{\bregs}{\mathit{bregs}}
\newcommand{\uregs}{\mathit{uregs}}


==> mprosper/_monitor-commands.tex <==
\newtheorem{preposition}{Proposition}
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}{Lemma}
\numberwithin{lemma}{section}



\newcommand{\SCTLR}{SCTLR}
\newcommand{\TTBRzero}{TTBR0}
\newcommand{\DACR}{DACR}
\newcommand{\Mem}{\texttt{mem}}
\newcommand{\PL}{\texttt{pl}}
\newcommand{\priv}{\mathit{mode}}
\newcommand{\regs}{\mathit{regs}}
\newcommand{\psrs}{\mathit{psrs}}
\newcommand{\coregs}{\mathit{coregs}}
\newcommand{\mem}{\mathit{mem}}
\newcommand{\accreq}{\mathit{accreq}}
\newcommand{\pgtype}{\mathit{pgtype}}
\newcommand{\pgrefs}{\mathit{pgrefs}}
\newcommand{\mode}{\mathit{mode}}
\newcommand{\refs}{\mathit{refs}}
\newcommand{\Data}{\mathit{D}}
\newcommand{\sound}{\mathit{sound}}
\newcommand{\type}{\mathit{type}}
\newcommand{\countt}{\mathit{count}}
\newcommand{\block}{\mathit{block}}
\newcommand{\fnsize}{\footnotesize \mathit{size}}
\newcommand{\fnref}{\footnotesize \mathit{ref}}
\newcommand{\relRule}[4]{\{#1:#2\to #3 \}}
\newcommand{\ineq}{$\neq$}
\newcommand{\negat}{$\neg$}
\newcommand{\fall}{$\forall$}
\newcommand{\impl}{$\Rightarrow$}
\newcommand{\sigmas}{$\sigma$}
\newcommand{\botm}{$\bot$}
\newcommand{\wrt}{\ensuremath{\texttt{write}_{32}}}
\newcommand{\rd}{\ensuremath{\texttt{read}_{32}}}
\newcommand{\mmu}[1]{\ensuremath{\texttt{mmu}_{#1}}}
\newcommand{\mathunderline}[2]{\ensuremath{\texttt{#1}_{#2}}}
\newcommand{\equivs}[1]{$\equiv_{#1}$}
\newcommand{\armv}{ARMv7}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\RealStateSpace}{\Sigma}
\newcommand{\ArmStateVar}{\sigma}
\newcommand{\UserMode}{PL0}
\newcommand{\KernelMode}{PL1}
\newcommand{\IdealStateSpace}{\mathcal{Q}}
\newcommand{\Exe}{\pi}
\newcommand{\mmudisbl}{\sigma.\SCTLR = 0}
\newcommand{\mmuenbl}{\sigma.\SCTLR \neq 0}
\newcommand{\descType}[3]{$#1(#2) = #3$}
\newcommand{\accPermChecker}[3]{#3(#1(#2))}
\newcommand{\RecCone}[1]{{#1}.c1}
\newcommand{\RecCtwo}[1]{{#1}.c2}
\newcommand{\RecMem}[1]{{#1}.mem}
\newcommand{\RecTTBR}[1]{{#1}.TTBR_{zero}}
\newcommand{\RecPgType}[1]{{#1}.\mathit{pgtype}}
\newcommand{\RecPgRefs}[1]{{#1}.rc}
\newcommand{\MaxRefCnt}{MAX}
\newcommand{\StaticMemType}{G_{mem}}
\newcommand{\MemTypeVar}{t}
\newcommand{\LOneSection}{SEC}
\newcommand{\LOnePt}{PT}
\newcommand{\SmallPageType}{SP}
\newcommand{\Types}[3]{#1 \vdash #2 : #3}
\newcommand{\inGuestMem}[1]{\Types \StaticMemType {#1} \GuestMemType}
\newcommand{\ptType}[3]{\Types {\RecPgType{#1}} {#2} {#3}}
\newcommand{\readDesc}[3]{$read_{#1}(#2, \sigma.mem, #3)$}
\newcommand{\readDescLOne}[3]{read_{L_1}(#1, #2, #3)}
\newcommand{\readDescLTwo}[3]{read_{L_2}(#1, #2, #3)}
\newcommand{\pgType}[1]{#1.type}
\newcommand{\pgAdd}[1]{#1.pa}
\newcommand{\pgPhBlock}[1]{#1.blk}
\newcommand{\secPhBlock}[1]{#1.sec}
\newcommand{\pgAP}[1]{#1.ap}
\newcommand{\funApl}[2]{$#1 #2$}
\newcommand{\Unmapped}{\bullet}
\newcommand{\HyperStateVar}{h}
\newcommand{\TlsStateVar}{s}
\newcommand{\PgTypeVar}{\tau}
\newcommand{\PgRefVar}{\rho}
\newcommand{\TlsState}[2]{\left \langle {#1},{#2} \right \rangle}

%rule for decreasing the reference counter
\newcommand{\refUpdateDec}[3]{\left\{\begin{array}{l l}
						#1(#2) - 1& #3\\
						#1(#2)\ & \mathit{otherwise}
					   \end{array}
					 \right.}					 
%rule for increasing the reference counter
\newcommand{\refUpdateInc}[3]{\left\{\begin{array}{l l}
						#1(#2)++ & #3\\
						#1(#2)\ & \mathit{otherwise}
					   \end{array}
					 \right.}
%rule for replacing part of the state
\newcommand{\replc}[2]{#1 := #2}

\newcommand{\LabelBlk}{\mathit{bl}}
\newcommand{\LabelVar}{\alpha}
\newcommand{\LabelUser}{0}
\newcommand{\LabelSwitchLOne}[1]{switchL1(#1)}
\newcommand{\LabelUnmapEntryLTwo}[2]{unmapEntryL2\tuple{#1, #2}}
\newcommand{\LabelMapLTwo}[4]{mapL2\tuple{#1, #2, #3, #4}}
\newcommand{\LabelCreateLOne}[1]{createL1(#1)}
\newcommand{\LabelCreateLTwo}[1]{createL2\(#1)}
\newcommand{\LabelFreeLOne}[1]{freeL1(#1)}
\newcommand{\LabelFreeLTwo}[1]{freeL2(#1)}
\newcommand{\LabelMapSecLOne}[1]{mapSecL1(#1)}
\newcommand{\LabelMapPtLOne}[1]{mapPtL1(#1)}
\newcommand{\LabelUnmapEntryLOne}[1]{unmapEntryL1(#1)}
\newcommand{\tlsTrans}[1]{\xrightarrow[]{#1}}
\newcommand{\inferTrans}[3]{#1 \tlsTrans{#2} #3}
\newcommand{\LTwoAP}[1]{l2\_acc\_perm(#1)}
\newcommand{\LOneSecAP}[1]{l1\_acc\_perm(#1)}
\newcommand{\MakeSPDesc}[2]{[#1,#2]}
\newcommand{\writeEntry}[4]{update\_entry(#1, #2, #3, #4)}
\newcommand{\ApGuestWritable}[1]{(0,wt) \in #1}
\newcommand{\ApGuestReadable}[1]{(0,rd) \in #1}
\newcommand{\OpLabel}[2]{\overset{#2}{#1}}
\newcommand{\TlsTrans}[1]{\OpLabel{\rightarrow}{#1}}
\newcommand{\MemTypeEquiv}[1]{\OpLabel{\equiv}{\StaticMemType:{#1}}}
\newcommand{\MemBlockUnchanged}[1]{\OpLabel{\equiv}{#1}}
\newcommand{\MmuEquiv}{\OpLabel{\equiv}{mmu}}
\newcommand{\Invariant}{\mathcal{I}}
\newcommand{\InvStates}{\mathcal{Q}_{\Invariant}}
\newcommand{\InvType}{\mathcal{I}_T}
\newcommand{\InvTypeOne}{\mathcal{I}_{T_1}}
\newcommand{\InvTypeTwo}{\mathcal{I}_{T_2}}
\newcommand{\InvRC}{\mathcal{I}_C}
\newcommand{\RcCount}{cnt}


==> tracklang.tex <==
%%
%% This is file `tracklang.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tracklang.dtx  (with options: `tracklang.tex,package')
%% 
%%  tracklang.dtx
%%  Copyright 2016 Nicola Talbot
%% 
%%  This work may be distributed and/or modified under the
%%  conditions of the LaTeX Project Public License, either version 1.3
%%  of this license of (at your option) any later version.
%%  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%%  and version 1.3 or later is part of all distributions of LaTeX
%%  version 2005/12/01 or later.
%% 
%%  This work has the LPPL maintenance status `maintained'.
%% 
%%  The Current Maintainer of this work is Nicola Talbot.
%% 
%%  This work consists of the files tracklang.dtx and tracklang.ins and the derived files tracklang.sty, tracklang.tex, tracklang-region-codes.tex, tracklang-scripts.sty, tracklang-scripts.tex.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% load packages that use tracklang for localisation
%% do code now to initialise
%% Pass all options to tracklang:
\ifnum\catcode`\@=11\relax
  \def\@tracklang@restore@at{}%
\else
  \expandafter\edef\csname @tracklang@restore@at\endcsname{%
    \noexpand\catcode`\noexpand\@=\number\catcode`\@\relax
  }%
 \catcode`\@=11\relax
\fi
\ifx\@tracklang@languages\undefined
\else
  \@tracklang@restore@at
  \expandafter\endinput
\fi
\expandafter\def\csname ver@tracklang.tex\endcsname{2016/11/03 v1.3.3
(NLCT) Track Languages Generic Code}
\long\def\@tracklang@ifundef#1#2#3{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  \else
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  \fi
}
\ifx\ifcsname\undefined
  \long\def\@tracklang@ifundef#1#2#3{%
    \expandafter\ifx\csname #1\endcsname\relax
      #2%
    \else
      #3%
    \fi
  }
\fi
\ifx\@@input\undefined
   \let\@tracklang@input\input
\else
   \let\@tracklang@input\@@input
\fi
\ifx\@nnil\undefined
  \def\@tracklang@nnil{\@nil}
\else
  \let\@tracklang@nnil\@nnil
\fi
\ifx\@for\undefined
  \long\def\@tracklang@for#1:=#2\do#3{%
    \expandafter\def\expandafter\@fortmp\expandafter{#2}%
    \ifx\@fortmp\empty
    \else
      \expandafter
        \@tracklang@forloop #2,\@nil,\@nil\@@ #1{#3}%
    \fi
  }
  \long\def\@tracklang@forloop#1,#2,#3\@@ #4#5{%
   \def #4{#1}%
   \ifx#4\@tracklang@nnil
   \else
     #5%
     \def #4{#2}%
     \ifx#4\@tracklang@nnil
     \else
       #5%
       \@tracklang@iforloop #3\@@ #4{#5}%
     \fi
   \fi
  }
  \long\def\@tracklang@iforloop#1,#2\@@ #3#4{%
    \def#3{#1}%
    \ifx#3\@tracklang@nnil
      \expandafter
        \@tracklang@fornoop
    \else
      #4\relax
      \expandafter\@tracklang@iforloop
    \fi
    #2\@@ #3{#4}%
  }
  \long\def\@tracklang@fornoop#1\@@ #2#3{}
\else
  \let\@tracklang@for\@for
\fi
\ifx\@namedef\undefined
  \def\@tracklang@namedef#1{\expandafter\def\csname#1\endcsname}
\else
  \let\@tracklang@namedef\@namedef
\fi
\def\@tracklang@enamedef#1{\expandafter\edef\csname#1\endcsname}
\def\@tracklang@nameuse#1{%
  \@tracklang@ifundef{#1}{}{\csname#1\endcsname}%
}
\ifx\@onelevel@sanitize\undefined
  \def\@tracklang@sanitize#1{%
    \edef#1{\expandafter\@tracklang@strip@prefix\meaning#1}%
  }
  \def\@tracklang@strip@prefix#1>{}
\else
  \let\@tracklang@sanitize\@onelevel@sanitize
\fi
\def\@tracklang@firstoftwo#1#2{#1}
\def\@tracklang@secondoftwo#1#2{#2}
\ifx\PackageError\undefined
  \def\@tracklang@err#1#2{%
    \errehelp{#2}%
    \errmessage{tracklang: #1}}
\else
  \def\@tracklang@err#1#2{\PackageError{tracklang}{#1}{#2}}
\fi
\newif\ifTrackLangShowWarnings
\TrackLangShowWarningstrue
\ifx\PackageWarning\undefined
  \def\@tracklang@warn#1{%
    \ifTrackLangShowWarnings
      {%
        \newlinechar=`\^^J
        \def\MessageBreak{^^J}%
        \message{^^Jtracklang Warning: #1 on line \the\inputlineno.^^J}%
      }%
    \fi
  }
\else
  \def\@tracklang@warn#1{%
    \ifTrackLangShowWarnings
      \PackageWarning{tracklang}{#1}%
    \fi
  }
\fi
\newif\ifTrackLangShowInfo
\TrackLangShowInfotrue
\ifx\PackageInfo\undefined
  \def\@tracklang@info#1{%
   \ifTrackLangShowInfo
     {%
       \newlinechar=`\^^J
       \def\MessageBreak{^^J}%
       \message{^^Jtracklang Info: #1 on line \the\inputlineno.^^J}%
     }%
   \fi
  }%
\else
  \def\@tracklang@info#1{%
    \ifTrackLangShowInfo
      \PackageInfo{tracklang}{#1}%
    \fi
  }%
\fi
\ifx\IfFileExists\undefined
 \long\def\@tracklang@IfFileExists#1#2#3{%
   \openin0=#1 %
   \ifeof0\relax
     \def\@tracklang@tmp{#3}%
   \else
     \closein0\relax
     \edef\@filef@und{#1 }%
     \def\@tracklang@tmp{#2}%
   \fi
   \@tracklang@tmp
 }

\else
  \let\@tracklang@IfFileExists\IfFileExists
\fi
\def\@tracklang@checklocale{%
  \ifx\TrackLangEnv\empty
  \else
    \ifx\TrackLangEnv\@tracklang@locale@posix
      \def\TrackLangEnv{}%
    \else
      \ifx\TrackLangEnv\@tracklang@locale@c
        \def\TrackLangEnv{}%
      \else
        \expandafter\@@tracklang@checklocale
           \TrackLangEnv\empty\relax
      \fi
    \fi
  \fi
}
\def\@@tracklang@checklocale#1#2\relax{%
  \ifx#1/\relax
    \def\TrackLangEnv{}%
  \fi
}
\def\@tracklang@locale@posix{POSIX}
\def\@tracklang@locale@c{C}
\ifx\directlua\undefined
  \def\@tracklang@tryshellescape#1{%
   \def\TrackLangQueryEnv{%
     \@tracklang@warn{\string\TrackLangQueryEnv\space
     non-operational as shell escape has been disabled}%
     \def\TrackLangEnv{}%
   }%
   \def\TrackLangQueryOtherEnv##1{%
     \@tracklang@warn{\string\TrackLangQueryOtherEnv{##1}\space
     non-operational as shell escape has been disabled}%
     \def\TrackLangEnv{}%
   }%
  }%
   \ifx\pdfshellescape\undefined
     \ifx\shellescape\undefined
        \def\@tracklang@tryshellescape#1{%
          \def\TrackLangQueryEnv{%
            \@tracklang@warn{\string\TrackLangQueryEnv\space
            non-operational as can't determine if the
            shell escape has been enabled. (Consider using
            eTeX or pdfTeX.)}%
            \def\TrackLangEnv{}%
          }%
          \def\TrackLangQueryOtherEnv##1{%
            \@tracklang@warn{\string\TrackLangQueryOtherEnv{##1}\space
            non-operational as can't determine if the
            shell escape has been enabled. (Consider using
            eTeX or pdfTeX.)}%
            \def\TrackLangEnv{}%
          }%
        }%
     \else
       \ifx\shellescape\relax
       \else
         \ifnum\shellescape=0\relax
         \else
           \def\@tracklang@tryshellescape#1{#1}%
         \fi
       \fi
     \fi
   \else
     \ifx\pdfshellescape\relax
       \ifx\shellescape\undefined
       \else
         \ifx\shellescape\relax
         \else
           \ifnum\shellescape=0\relax
           \else
             \def\@tracklang@tryshellescape#1{#1}%
           \fi
         \fi
       \fi
     \else
       \ifnum\pdfshellescape=0\relax
       \else
         \def\@tracklang@tryshellescape#1{#1}%
       \fi
     \fi
   \fi
   \@tracklang@tryshellescape
   {%
     \def\TrackLangQueryEnv{%
       \begingroup\endlinechar=-1\relax
       \everyeof{\noexpand}%
       \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
         \@tracklang@input|"kpsewhich --var-value LC_ALL" }}\x
       \@tracklang@checklocale
       \ifx\TrackLangEnv\empty
         \begingroup\endlinechar=-1\relax
         \everyeof{\noexpand}%
         \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
           \@tracklang@input|"kpsewhich --var-value LANG" }}\x
         \@tracklang@checklocale
         \ifx\TrackLangEnv\empty
           \ifx\TeXOSQueryLocale\undefined
             \@tracklang@warn{Locale environment variables
              unavailable (tried LC\string_ALL and LANG)}%
           \else
             \@tracklang@info{Using texosquery to find locale}%
             \TeXOSQueryLocale\TrackLangEnv
             \ifx\TrackLangEnv\empty
               \@tracklang@warn{Locale can't be found
               (tried querying LC\string_ALL and LANG variables and
               tried using texosquery)}%
             \fi
           \fi
         \fi
       \fi
     }%
     \def\TrackLangQueryOtherEnv#1{%
       \begingroup\endlinechar=-1\relax
       \everyeof{\noexpand}%
       \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
         \@tracklang@input|"kpsewhich --var-value LC_ALL" }}\x
       \@tracklang@checklocale
       \ifx\TrackLangEnv\empty
         \begingroup\endlinechar=-1\relax
         \everyeof{\noexpand}%
         \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
           \@tracklang@input|"kpsewhich --var-value #1" }}\x
         \@tracklang@checklocale
         \ifx\TrackLangEnv\empty
           \begingroup\endlinechar=-1\relax
           \everyeof{\noexpand}%
           \edef\x{\endgroup\def\noexpand\TrackLangEnv{%
             \@tracklang@input|"kpsewhich --var-value LANG"}}\x
           \@tracklang@checklocale
           \ifx\TrackLangEnv\empty
             \ifx\TeXOSQueryLocale\undefined
             \@tracklang@warn{Locale environment variables unavailable
              (tried LC\string_ALL, #1 and LANG)}%
             \else
               \@tracklang@info{Using texosquery to find locale}%
               \TeXOSQueryLocale\TrackLangEnv
               \ifx\TrackLangEnv\empty
                 \@tracklang@warn{Locale can't be found
                 (tried querying LC\string_ALL, #1 and LANG variables and
                 tried using texosquery)}%
               \fi
             \fi
           \fi
         \fi
       \fi
     }%
  }%
\else
   \def\TrackLangQueryEnv{%
     \edef\TrackLangEnv{\directlua{
       l = os.getenv("LC_ALL")
       if l == nil or l == "" or l == "C" or l == "POSIX"
                   or string.find(l, "^/") then
         l = os.getenv("LANG")
         if l == nil or l == "" or l == "C" or l == "POSIX"
                     or string.find(l, "^/") then
           l=os.setlocale(nil)
           if l == nil or l == "C" or l == "POSIX"
                       or string.find(l, "^/") then
             l = ""
           end
         end
       end
       tex.print(l)}}%
       \ifx\TrackLangEnv\empty
         \ifx\TeXOSQueryLocale\undefined
         \@tracklang@warn{Locale can't be found through Lua
          (tried querying LC\string_ALL and LANG variables and
           os.setlocale(nil))}%
         \else
           \TeXOSQueryLocale\TrackLangEnv
           \ifx\TrackLangEnv\empty
             \@tracklang@warn{Locale can't be found through Lua
             (tried querying LC\string_ALL and LANG variables and
             os.setlocale(nil) and tried using texosquery)}%
           \fi
         \fi
       \fi
   }
   \def\TrackLangQueryOtherEnv#1{%
     \edef\TrackLangEnv{\directlua{
       l = os.getenv("LC_ALL")
       if l == nil or l == "" or l == "C" or l == "POSIX"
                   or string.find(l, "^/") then
         l = os.getenv("#1")
         if l == nil or l == "" or l == "C" or l == "POSIX"
                     or string.find(l, "^/") then
           l = os.getenv("LANG")
           if l == nil or l == "" or l == "C" or l == "POSIX"
                       or string.find(l, "^/") then
             l=os.setlocale(nil)
             if l == nil or l == "C" or l == "POSIX"
                         or string.find(l, "^/") then
               l = ""
             end
           end
         end
       end
       tex.print(l}}%
       \ifx\TrackLangEnv\empty
         \ifx\TeXOSQueryLocale\undefined
         \@tracklang@warn{Locale can't be found through Lua
          (tried querying LC\string_ALL, #1 and LANG variables and
           os.setlocale(nil))}%
         \else
           \TeXOSQueryLocale\TrackLangEnv
           \ifx\TrackLangEnv\empty
             \@tracklang@warn{Locale can't be found through Lua
             (tried querying LC\string_ALL, #1 and LANG variables and
             os.setlocale(nil) and tried using texosquery)}%
           \fi
         \fi
       \fi
   }
\fi
\def\TrackLangParseFromEnv{%
  \ifx\TrackLangEnv\undefined
     \@tracklang@warn{\string\TrackLangParseFromEnv\space
     non-operational as \string\TrackLangEnv\space hasn't been
     defined}%
     \def\TrackLangEnvLang{}%
     \def\TrackLangEnvTerritory{}%
     \def\TrackLangEnvCodeSet{}%
     \def\TrackLangEnvModifier{}%
  \else
    \ifx\TrackLangEnv\empty
      \@tracklang@warn{\string\TrackLangParseFromEnv\space
      non-operational as \string\TrackLangEnv\space is empty}%
      \def\TrackLangEnvLang{}%
      \def\TrackLangEnvTerritory{}%
      \def\TrackLangEnvCodeSet{}%
      \def\TrackLangEnvModifier{}%
    \else
      \@tracklang@parse@locale{\TrackLangEnv}%
      \let\TrackLangEnvLang\@TrackLangEnvLang
      \let\TrackLangEnvTerritory\@TrackLangEnvTerritory
      \let\TrackLangEnvCodeSet\@TrackLangEnvCodeSet
      \let\TrackLangEnvModifier\@TrackLangEnvModifier
    \fi
  \fi
}
\def\@tracklang@parse@locale#1{%
  \def\@TrackLangEnvLang{}%
  \def\@TrackLangEnvSubLang{}%
  \def\@TrackLangEnvFirstSubLang{}%
  \def\@TrackLangEnvTerritory{}%
  \def\@TrackLangEnvCodeSet{}%
  \def\@TrackLangEnvVariant{}%
  \def\@TrackLangEnvModifier{}%
  \def\@TrackLangEnvScript{}%
  \def\@TrackLangEnvAdditional{}%
  \expandafter\ifx\expandafter\relax#1\relax
  \else
    \expandafter\@tracklang@parseenv
      #1..\relax\@tracklang@end@parseenv\@tracklang@result
    \ifx\@tracklang@result\empty
    \else
      \expandafter\@tracklang@split@underscoreorhyp\expandafter
       {\@tracklang@result}%
      \let\@TrackLangEnvLang\@tracklang@split@pre
      \let\@TrackLangEnvTerritory\@tracklang@split@post
    \fi
  \fi
}
\def\@tracklang@split@underscoreorhyp#1{%
  \@tracklang@split@underscore{#1}%
  \ifx\@tracklang@split@post\empty
    \@tracklang@split@hyphen{#1}%
    \ifx\@tracklang@split@post\empty
      \@tracklang@split@otherunderscore{#1}%
    \fi
  \fi
}
{
  \catcode`\_8\relax
  \gdef\@tracklang@split@underscore#1{%
    \@@tracklang@split@underscore#1__\relax\@tracklang@end@split@underscore
  }
  \gdef\@@tracklang@split@underscore#1_#2_#3\@tracklang@end@split@underscore{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@underscore@remainder#2_#3%
    \fi
  }
  \gdef\@tracklang@split@underscore@remainder#1__\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
{
  \catcode`\_12\relax
  \gdef\@tracklang@split@otherunderscore#1{%
    \@@tracklang@split@otherunderscore#1__\relax\@tracklang@end@split@underscore
  }
  \gdef\@@tracklang@split@otherunderscore#1_#2_#3\@tracklang@end@split@underscore{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@otherunderscore@remainder#2_#3%
    \fi
  }
  \gdef\@tracklang@split@otherunderscore@remainder#1__\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
{
  \catcode`\-12\relax
  \gdef\@tracklang@split@hyphen#1{%
    \@@tracklang@split@hyphen#1--\relax\@tracklang@end@split@hyphen
  }
  \gdef\@@tracklang@split@hyphen#1-#2-#3\@tracklang@end@split@hyphen{%
    \def\@tracklang@split@pre{#1}%
    \ifx\relax#3\relax
      \def\@tracklang@split@post{#2}%
    \else
      \@tracklang@split@hyphen@remainder#2-#3%
    \fi
  }
  \gdef\@tracklang@split@hyphen@remainder#1--\relax{%
    \def\@tracklang@split@post{#1}%
  }
}
\gdef\@tracklang@parseenv#1.#2.#3\@tracklang@end@parseenv#4{%
  \def\@TrackLangEnvCodeSet{#2}%
  \def#4{#1}%
  \ifx\@TrackLangEnvCodeSet\empty
    \tracklangparsemod#4%
  \else
    \tracklangparsemod\@TrackLangEnvCodeSet
  \fi
}
{\catcode`\@=12\relax
  \gdef\tracklangparsemod#1{
    \expandafter\tracklangparseenvatmod#1@@\relax\tracklangendparseenvatmod
    \let#1\tracklangtmp
  }%
  \gdef\tracklangparseenvatmod#1@#2@#3\tracklangendparseenvatmod{%
    \def\tracklangtmp{#1}%
    \expandafter\def\csname @TrackLangEnvModifier\endcsname{#2}%
    \csname @tracklang@sanitize\expandafter\endcsname
      \csname @TrackLangEnvModifier\endcsname
  }
}
\def\@tracklang@languages{}
\def\@tracklang@dialects{}
\def\@tracklang@ifinlist#1#2#3#4{%
  \def\@tracklang@doifinlist##1,#1,##2\end@tracklang@doifinlist{%
     \def\@before{##1}%
     \def\@after{##2}%
  }%
  \expandafter\@tracklang@doifinlist\expandafter,#2,#1,\@nil
    \end@tracklang@doifinlist
  \ifx\@after\@tracklang@nnil
    #4%
  \else
    #3%
  \fi
}
\def\@tracklang@add#1#2{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}#2%
    {%
    }%
    {%
     \ifx\empty#2\relax
       \let#2\@tracklang@element
     \else
       \edef#2{#2,\@tracklang@element}%
     \fi
    }%
  \fi
}
\def\AddTrackedDialect#1#2{%
 \@tracklang@add{#1}{\@tracklang@dialects}%
 \@tracklang@add{#2}{\@tracklang@languages}%
 \@tracklang@enamedef{@tracklang@fromdialect@#1}{#2}%
 \@tracklang@ifundef{@tracklang@todialect@#2}%
 {\@tracklang@enamedef{@tracklang@todialect@#2}{#1}}%
 {%
   \def\@tracklang@lang{#1}%
   \expandafter\@tracklang@add\expandafter\@tracklang@lang
     \csname @tracklang@todialect@#2\endcsname
 }%
 \edef\TrackLangLastTrackedDialect{#1}%
}
\def\AddTrackedLanguage#1{%
  \AddTrackedDialect{#1}{#1}%
}
\def\@tracklang@known@langs{}
\def\TrackLangNewLanguage#1#2#3#4#5#6#7{%
 \@tracklang@add{#1}{\@tracklang@known@langs}%
 \edef\@tracklang@tmp{#2}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#2}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@1@#1}{#2}%
 \fi
 \edef\@tracklang@tmp{#3}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#3}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@2@#1}{#3}%
 \fi
 \edef\@tracklang@tmp{#4}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@639@2B@#1}{#4}%
 \fi
 \edef\@tracklang@tmp{#5}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knownisolang@#5}{#1}%
   \@tracklang@enamedef{@tracklang@knowniso@639@3@#1}{#5}%
 \fi
 \edef\@tracklang@tmp{#6}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@3166@#1}{#6}%
 \fi
 \edef\@tracklang@tmp{#7}%
 \ifx\@tracklang@tmp\empty
 \else
   \@tracklang@enamedef{@tracklang@knowniso@script@#1}{#7}%
 \fi
}
\def\TrackLangIfKnownLang#1#2#3{%
  \expandafter\@tracklang@ifinlist\expandafter{#1}{\@tracklang@known@langs}%
  {#2}%
  {#3}%
}
\def\TrackLangIfKnownIsoTwoLetterLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@1@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoTwoLetterLang#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@1@#1}%
}
\def\TrackLangIfKnownIsoThreeLetterLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@2@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoThreeLetterLang#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@2@#1}%
}
\def\TrackLangIfKnownIsoThreeLetterLangB#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@639@2B@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownIsoThreeLetterLangB#1{%
  \@tracklang@nameuse{@tracklang@knowniso@639@2B@#1}%
}
\def\TrackLangIfKnownLangFromIso#1#2#3{%
  \@tracklang@ifundef{@tracklang@knownisolang@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownLangFromIso#1{%
  \@tracklang@nameuse{@tracklang@knownisolang@#1}%
}
\def\TrackLangIfHasKnownCountry#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@3166@#1}%
  {#3}%
  {#2}%
}
\def\TrackLangGetKnownCountry#1{%
  \@tracklang@nameuse{@tracklang@knowniso@3166@#1}%
}
\def\TrackLangGetDefaultScript#1{%
  \@tracklang@nameuse{@tracklang@knowniso@script@#1}%
}
\def\TrackLangIfHasDefaultScript#1#2#3{%
  \@tracklang@ifundef{@tracklang@knowniso@script@#1}{#3}{#2}%
}
\def\AddTrackedIsoLanguage#1#2#3{%
  \@tracklang@enamedef{@tracklang@#1@isofromlang@#3}{#2}%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}%
  {\@tracklang@enamedef{@tracklang@#1@isotolang@#2}{#3}}%
  {%
    \def\@tracklang@lang{#3}%
    \expandafter\@tracklang@add\expandafter\@tracklang@lang
      \csname @tracklang@#1@isotolang@#2\endcsname
  }%
}
\def\TrackedLanguageFromIsoCode#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isotolang@#2}%
}
\def\TrackedIsoCodeFromLanguage#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isofromlang@#2}%
}
\def\TrackedLanguageFromDialect#1{%
 \@tracklang@nameuse{@tracklang@fromdialect@#1}%
}
\def\TrackedDialectsFromLanguage#1{%
 \@tracklang@nameuse{@tracklang@todialect@#1}%
}
\def\TwoLetterIsoCountryCode{3166-1}
\def\TwoLetterIsoLanguageCode{639-1}
\def\ThreeLetterIsoLanguageCode{639-2}
\def\ThreeLetterExtIsoLanguageCode{639-3}
\def\SetTrackedDialectModifier#1#2{%
  \@tracklang@enamedef{@tracklang@modifier@#1}{#2}%
}
\def\GetTrackedDialectModifier#1{%
  \@tracklang@nameuse{@tracklang@modifier@#1}%
}
\def\IfHasTrackedDialectModifier#1#2#3{%
  \@tracklang@ifundef{@tracklang@modifier@#1}{#3}{#2}%
}
\def\SetTrackedDialectScript#1#2{%
  \@tracklang@enamedef{@tracklang@script@#1}{#2}%
}
\def\GetTrackedDialectScript#1{%
  \@tracklang@nameuse{@tracklang@script@#1}%
}
\def\IfHasTrackedDialectScript#1#2#3{%
  \@tracklang@ifundef{@tracklang@script@#1}{#3}{#2}%
}
\def\IfTrackedDialectIsScriptCs#1#2#3#4{%
  \IfHasTrackedDialectScript{#1}%
  {%
    \expandafter\ifx\expandafter#2\csname @tracklang@script@#1\endcsname
      #3%
    \else
      #4%
    \fi
  }%
  {%
    \TrackLangIfHasDefaultScript{\TrackedLanguageFromDialect{#1}}%
    {%
      \expandafter\ifx\expandafter
        #2\csname @tracklang@knowniso@script@\TrackedLanguageFromDialect{#1}\endcsname
         #3%
      \else
         #4%
      \fi
    }%
    {#4}%
  }%
}
\def\SetTrackedDialectVariant#1#2{%
  \@tracklang@enamedef{@tracklang@variant@#1}{#2}%
}
\def\GetTrackedDialectVariant#1{%
  \@tracklang@nameuse{@tracklang@variant@#1}%
}
\def\IfHasTrackedDialectVariant#1#2#3{%
  \@tracklang@ifundef{@tracklang@variant@#1}{#3}{#2}%
}
\def\SetTrackedDialectSubLang#1#2{%
  \@tracklang@enamedef{@tracklang@sublang@#1}{#2}%
}
\def\GetTrackedDialectSubLang#1{%
  \@tracklang@nameuse{@tracklang@sublang@#1}%
}
\def\IfHasTrackedDialectSubLang#1#2#3{%
  \@tracklang@ifundef{@tracklang@sublang@#1}{#3}{#2}%
}
\def\SetTrackedDialectAdditional#1#2{%
  \@tracklang@enamedef{@tracklang@extra@#1}{#2}%
}
\def\GetTrackedDialectAdditional#1{%
  \@tracklang@nameuse{@tracklang@extra@#1}%
}
\def\IfHasTrackedDialectAdditional#1#2#3{%
  \@tracklang@ifundef{@tracklang@extra@#1}{#3}{#2}%
}
\def\GetTrackedLanguageTag#1{%
  \IfTrackedLanguageHasIsoCode{639-1}{\TrackedLanguageFromDialect{#1}}%
  {\TrackedIsoCodeFromLanguage{639-1}{\TrackedLanguageFromDialect{#1}}}%
  {%
    \IfTrackedLanguageHasIsoCode{639-2}{\TrackedLanguageFromDialect{#1}}%
    {\TrackedIsoCodeFromLanguage{639-2}{\TrackedLanguageFromDialect{#1}}}%
    {%
      \IfTrackedLanguageHasIsoCode{639-3}{\TrackedLanguageFromDialect{#1}}%
      {\TrackedIsoCodeFromLanguage{639-3}{\TrackedLanguageFromDialect{#1}}}%
      {und}% undefined
    }%
  }%
  \@tracklang@ifundef{@tracklang@sublang@#1}%
  {}%
  {-\csname @tracklang@sublang@#1\endcsname}%
  \@tracklang@ifundef{@tracklang@script@#1}%
  {}%
  {-\csname @tracklang@script@#1\endcsname}%
  \IfTrackedLanguageHasIsoCode{3166-1}{#1}%
  {-\TrackedIsoCodeFromLanguage{3166-1}{#1}}%
  {}%
  \@tracklang@ifundef{@tracklang@variant@#1}%
  {}%
  {-\csname @tracklang@variant@#1\endcsname}%
  \@tracklang@ifundef{@tracklang@extra@#1}%
  {}%
  {-\csname @tracklang@extra@#1\endcsname}%
}
\def\SetCurrentTrackedDialect#1{%
  \edef\CurrentTrackedDialect{#1}%
  \IfTrackedDialect{\CurrentTrackedDialect}%
  {}%
  {%
    \IfHookHasMappingFromTrackedDialect{\CurrentTrackedDialect}%
    {%
      \IfTrackedDialect{\GetTrackedDialectFromMapping\CurrentTrackedDialect}%
      {%
        \edef\CurrentTrackedDialect{\GetTrackedDialectFromMapping
          {\CurrentTrackedDialect}}%
      }%
      {%
        \IfTrackedLanguage{#1}%
        {%
          \edef\@tracklang@dialects{\TrackedDialectsFromLanguage{#1}}%
          \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
            \let\CurrentTrackedDialect\@tracklang@dialect
          }%
        }%
        {}%
      }%
    }%
    {%
      \IfTrackedLanguage{#1}%
      {%
        \edef\@tracklang@dialects{\TrackedDialectsFromLanguage{#1}}%
        \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
          \let\CurrentTrackedDialect\@tracklang@dialect
        }%
      }%
      {}%
    }%
  }%
  \IfTrackedDialect{\CurrentTrackedDialect}%
  {%
    \edef\CurrentTrackedLanguage{%
      \TrackedLanguageFromDialect{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectModifier{%
      \GetTrackedDialectModifier{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectVariant{%
      \GetTrackedDialectVariant{\CurrentTrackedDialect}}%
    \IfHasTrackedDialectScript{\CurrentTrackedDialect}%
    {%
      \edef\CurrentTrackedDialectScript{%
        \GetTrackedDialectScript{\CurrentTrackedDialect}}%
    }%
    {%
      \edef\CurrentTrackedDialectScript{%
        \TrackLangGetDefaultScript\CurrentTrackedLanguage}%
    }%
    \edef\CurrentTrackedDialectSubLang{%
      \GetTrackedDialectSubLang{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedDialectAdditional{%
      \GetTrackedDialectAdditional{\CurrentTrackedDialect}}%
    \edef\CurrentTrackedLanguageTag{%
      \GetTrackedLanguageTag{\CurrentTrackedDialect}}%
    \IfTrackedLanguageHasIsoCode{3166-1}{\CurrentTrackedDialect}%
    {%
      \edef\CurrentTrackedRegion{%
       \TrackedIsoCodeFromLanguage{3166-1}{\CurrentTrackedDialect}}%
    }%
    {\def\CurrentTrackedRegion{}}%
    \IfTrackedLanguageHasIsoCode{639-1}{\CurrentTrackedLanguage}%
    {%
      \edef\CurrentTrackedIsoCode{%
       \TrackedIsoCodeFromLanguage{639-1}{\CurrentTrackedLanguage}}%
    }%
    {%
      \IfTrackedLanguageHasIsoCode{639-2}{\CurrentTrackedLanguage}%
      {%
        \edef\CurrentTrackedIsoCode{%
         \TrackedIsoCodeFromLanguage{639-2}{\CurrentTrackedLanguage}}%
      }%
      {%
        \IfTrackedLanguageHasIsoCode{639-3}{\CurrentTrackedLanguage}%
        {%
          \edef\CurrentTrackedIsoCode{%
           \TrackedIsoCodeFromLanguage{639-3}{\CurrentTrackedLanguage}}%
        }%
        {%
          \def\CurrentTrackedIsoCode{}%
        }%
      }%
    }%
  }%
  {%
    \@tracklang@warn{Unknown dialect label `#1' passed to
      \string\SetCurrentTrackedDialect}%
    \edef\CurrentTrackedLanguage{\languagename}%
    \def\CurrentTrackedDialectModifier{}%
    \def\CurrentTrackedDialectVariant{}%
    \def\CurrentTrackedDialectScript{}%
    \def\CurrentTrackedDialectSubLang{}%
    \def\CurrentTrackedDialectAdditional{}%
    \def\CurrentTrackedIsoCode{}%
    \def\CurrentTrackedRegion{}%
    \def\CurrentTrackedLanguageTag{und}%
  }%
}
\def\AddTrackedLanguageIsoCodes#1{%
  \@tracklang@ifundef{@tracklang@knowniso@639@1@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\TwoLetterIsoLanguageCode
      {\csname @tracklang@knowniso@639@1@#1\endcsname}{#1}%
  }%
  \@tracklang@ifundef{@tracklang@knowniso@639@2@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\ThreeLetterIsoLanguageCode
       {\csname @tracklang@knowniso@639@2@#1\endcsname}{#1}%
    \@tracklang@ifundef{@tracklang@knowniso@639@2B@#1}%
    {}%
    {%
      \AddTrackedIsoLanguage{\ThreeLetterIsoLanguageCode-T}%
         {\csname @tracklang@knowniso@639@2@#1\endcsname}{#1}%
      \AddTrackedIsoLanguage{\ThreeLetterIsoLanguageCode-B}%
         {\csname @tracklang@knowniso@639@2B@#1\endcsname}{#1}%
    }%
  }%
  \@tracklang@ifundef{@tracklang@knowniso@639@3@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage\ThreeLetterExtIsoLanguageCode
      {\csname @tracklang@knowniso@639@3@#1\endcsname}{#1}%
  }%
}
\def\AddTrackedCountryIsoCode#1{%
  \@tracklang@ifundef{@tracklang@knowniso@3166@#1}%
  {}%
  {%
    \AddTrackedIsoLanguage{3166-1}%
      {\csname @tracklang@knowniso@3166@#1\endcsname}{#1}%
  }%
}
\def\TrackPredefinedDialect#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \@tracklang@err{Dialect or language `#1' is not predefined}{}%
  }%
  {\@tracklang@nameuse{@tracklang@add@#1}}%
}
\def\@tracklang@hassecondchar#1#2\@end@tracklang@hassecondchar#3#4{%
  \ifx\relax#2\relax
    #4%
  \else
    #3%
  \fi
}
\def\@tracklang@hasthirdchar#1#2#3\@end@tracklang@hasthirdchar#4#5{%
  \ifx\relax#3\relax
    #5%
  \else
    #4%
  \fi
}
\def\@tracklang@hasfourthchar#1#2#3#4\@end@tracklang@hasfourthchar#5#6{%
  \ifx\relax#4\relax
    #6%
  \else
    #5%
  \fi
}
\def\@tracklang@hasfifthchar#1#2#3#4#5\@end@tracklang@hasfifthchar#6#7{%
  \ifx\relax#5\relax
    #7%
  \else
    #6%
  \fi
}
\def\@tracklang@hasninthchar#1#2#3#4#5#6#7#8#9\@end@tracklang@hasninthchar{%
  \ifx\relax#9\relax
    \expandafter\@tracklang@secondoftwo
  \else
    \expandafter\@tracklang@firstoftwo
  \fi
}
\def\@tracklang@ifalpha#1#2#3{%
  \ifx\relax#1\relax
    #3%
  \else
   \ifnum\lccode`#1<`a\relax
     #3%
   \else
     \ifnum\lccode`#1>`z\relax
      #3%
     \else
       #2%
     \fi
   \fi
  \fi
}
\def\@tracklang@ifdigit#1#2#3{%
  \ifx\relax#1\relax
    #3%
  \else
   \ifnum`#1<`0\relax
     #3%
   \else
     \ifnum`#1>`9\relax
      #3%
     \else
       #2%
     \fi
   \fi
  \fi
}
\def\@tracklang@ifalldigits#1{%
 \expandafter\ifx\relax#1\relax
   \expandafter\@tracklang@secondoftwo
 \else
   \expandafter\@@tracklang@ifalldigits#1\@tracklang@nnil
 \fi
}
\def\@@tracklang@ifalldigits#1{%
  \ifx#1\@tracklang@nnil
   \def\@tracklang@next{\expandafter\@tracklang@firstoftwo}%
  \else
    \@tracklang@ifdigit{#1}%
    {%
      \let\@tracklang@next\@@tracklang@ifalldigits
    }%
    {%
      \def\@tracklang@next##1\@tracklang@nnil{%
        \expandafter\@tracklang@secondoftwo}%
    }%
  \fi
  \@tracklang@next
}
\def\@tracklang@ifalphanumeric#1#2#3{%
  \@tracklang@ifalpha{#1}%
  {#2}%
  {%
    \@tracklang@ifdigit{#1}{#2}{#3}%
  }%
}
\def\TrackLangIfAlphaNumericChar#1#2#3{%
  \expandafter\ifx\expandafter\relax#1\relax
    #3%
  \else
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {#3}%
    {\expandafter\@tracklang@ifalphanumeric#1{#2}{#3}}%
  \fi
}
\def\TrackLangIfLanguageTag#1#2#3{%
  \expandafter\@tracklang@hasthirdchar#1\relax\relax\relax
    \@end@tracklang@hasthirdchar
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\@end@tracklang@hasfourthchar
    {#3}%
    {%
     \expandafter\@tracklang@iflanguage@iii@tag#1{#2}{#3}%
    }%
  }%
  {%
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {%
     \expandafter\@tracklang@iflanguage@ii@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@iflanguage@ii@tag#1#2#3#4{%
  \ifnum\lccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      #3%
    \else
      #4%
    \fi
  \else
    #4%
  \fi
}
\def\@tracklang@iflanguage@iii@tag#1#2#3#4#5{%
  \ifnum\lccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      \ifnum\lccode`#3=`#3\relax
        #4%
      \else
        #5%
      \fi
    \else
      #5%
    \fi
  \else
    #5%
  \fi
}
\def\TrackLangIfRegionTag#1#2#3{%
  \expandafter\@tracklang@hasthirdchar#1\relax\relax\relax
    \@end@tracklang@hasthirdchar
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\@end@tracklang@hasfourthchar
    {%
      #3%
    }%
    {%
      \@tracklang@ifalldigits{#1}{#2}{#3}%
    }%
  }%
  {%
    \expandafter\@tracklang@hassecondchar#1\relax\relax
      \@end@tracklang@hassecondchar
    {%
     \expandafter\@tracklang@ifregion@ii@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifregion@ii@tag#1#2#3#4{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\uccode`#2=`#2\relax
      #3%
    \else
      #4%
    \fi
  \else
    #4%
  \fi
}
\def\@tracklang@ifregion@iii@tag#1#2#3#4#5{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\uccode`#2=`#2\relax
      \ifnum\uccode`#3=`#3\relax
        #4%
      \else
        #5%
      \fi
    \else
      #5%
    \fi
  \else
    #5%
  \fi
}
\def\TrackLangIfScriptTag#1#2#3{%
  \expandafter\@tracklang@hasfifthchar#1\relax\relax\relax\relax\relax
    \@end@tracklang@hasfifthchar
  {#3}%
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\relax\relax\relax
      \@end@tracklang@hasfourthchar
    {%
     \expandafter\@tracklang@ifscripttag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifscripttag#1#2#3#4#5#6{%
  \ifnum\uccode`#1=`#1\relax
    \ifnum\lccode`#2=`#2\relax
      \ifnum\lccode`#3=`#3\relax
        \ifnum\lccode`#4=`#4\relax
          #5%
        \else
          #6%
        \fi
      \else
        #6%
      \fi
    \else
      #6%
    \fi
  \else
    #6%
  \fi
}
\def\TrackLangIfVariantTag#1#2#3{%
  \expandafter\@tracklang@hasfifthchar#1\relax\relax\relax\relax\relax
    \@end@tracklang@hasfifthchar
  {%
    \expandafter\@tracklang@hasninthchar#1\relax\relax\relax\relax\relax
      \relax\relax\relax\relax
      \@end@tracklang@hasninthchar
    {#3}%
    {#2}%
  }%
  {%
    \expandafter\@tracklang@hasfourthchar#1\relax\relax\relax\relax
      \@end@tracklang@hasfourthchar
    {%
      \expandafter\@tracklang@ifvariant@iv@tag#1{#2}{#3}%
    }%
    {#3}%
  }%
}
\def\@tracklang@ifvariant@iv@tag#1#2#3#4#5#6{%
  \@tracklang@ifdigit{#1}%
  {#5}
  {#6}%
}
\def\@tracklang@parse@extlang{%
   \TrackLangIfLanguageTag{\@tracklang@split@pre}
   {%
     \ifx\@TrackLangEnvSubLang\empty
       \let\@TrackLangEnvSubLang\@tracklang@split@pre
       \let\@TrackLangEnvFirstSubLang\@TrackLangEnvSubLang
     \else
       \edef\@TrackLangEnvSubLang{\@TrackLangEnvSubLang-\@tracklang@split@pre}%
     \fi
     \ifx\@tracklang@split@post\empty
     \else
       \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
       \ifx\@tracklang@split@pre\empty
       \else
         \@tracklang@parse@extlang
       \fi
     \fi
   }%
   {}%
}
\def\@tracklang@parse@variant{%
   \TrackLangIfVariantTag{\@tracklang@split@pre}
   {%
     \ifx\@TrackLangEnvVariant\empty
       \let\@TrackLangEnvVariant\@tracklang@split@pre
     \else
       \edef\@TrackLangEnvVariant{\@TrackLangEnvVariant
         -\@tracklang@split@pre}%
     \fi
     \ifx\@tracklang@split@post\empty
     \else
       \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
       \ifx\@tracklang@split@pre\empty
       \else
         \@tracklang@parse@variant
       \fi
     \fi
   }%
   {}%
}
\def\TrackLanguageTag#1{%
  \edef\@tracklang@tag{#1}%
  \ifx\@tracklang@tag\empty
    \@tracklang@warn{Empty tag in \string\TrackLanguageTag}%
  \else
    \expandafter\@TrackLanguageTag\expandafter{\@tracklang@tag}%
  \fi
}
\def\@TrackLanguageTag#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
     \@tracklang@parselangtag{#1}%
     \@tracklang@track@locale
  }%
  {%
    \@tracklang@nameuse{@tracklang@add@#1}%
  }%
}
\def\@tracklang@parselangtag#1{%
  \def\@TrackLangEnvLang{}%
  \def\@TrackLangEnvSubLang{}%
  \def\@TrackLangEnvFirstSubLang{}%
  \def\@TrackLangEnvTerritory{}%
  \def\@TrackLangEnvCodeSet{}%
  \def\@TrackLangEnvVariant{}%
  \def\@TrackLangEnvModifier{}%
  \def\@TrackLangEnvScript{}%
  \def\@TrackLangEnvAdditional{}%
  \@tracklang@split@underscoreorhyp{#1}%
  \let\@TrackLangEnvLang\@tracklang@split@pre
  \ifx\@tracklang@split@post\empty
  \else
     \expandafter\@tracklang@split@underscoreorhyp\expandafter
       {\@tracklang@split@post}%
     \@tracklang@parse@extlang
     \TrackLangIfScriptTag{\@tracklang@split@pre}%
     {%
       \let\@TrackLangEnvScript\@tracklang@split@pre
       \ifx\@tracklang@split@post\empty
       \else
         \expandafter\@tracklang@split@underscoreorhyp\expandafter
           {\@tracklang@split@post}%
       \fi
     }%
     {}%
     \TrackLangIfRegionTag{\@tracklang@split@pre}%
     {%
       \expandafter\@tracklang@hasthirdchar\@tracklang@split@pre
          \relax\relax\relax
          \@end@tracklang@hasthirdchar
       {%
         \ifx\TrackLangIfKnownNumericRegion\undefined
           \@tracklang@input tracklang-region-codes.tex
         \fi
         \TrackLangIfKnownNumericRegion{\@tracklang@split@pre}%
         {%
           \edef\@TrackLangEnvTerritory{%
             \TrackLangNumericToAlphaIIRegion{\@tracklang@split@pre}%
           }%
         }%
         {%
           \let\@TrackLangEnvTerritory\@tracklang@split@pre
           \@tracklang@warn{Unrecognised numeric region code
             `\@tracklang@split@pre'}%
         }%
       }%
       {%
         \let\@TrackLangEnvTerritory\@tracklang@split@pre
       }%
     \expandafter\@tracklang@split@underscoreorhyp\expandafter
         {\@tracklang@split@post}%
     }%
     {}%
     \@tracklang@parse@variant
     \let\@TrackLangEnvAdditional\@tracklang@split@post
  \fi
}%
\def\GetTrackedDialectFromLanguageTag#1#2{%
  \def#2{}%
  \@tracklang@parselangtag{#1}%
  \edef\@tracklang@dialect{%
   \@TrackLangEnvLang
   \@TrackLangEnvSubLang
   \@TrackLangEnvScript
   \@TrackLangEnvTerritory
   \@TrackLangEnvModifier
   \@TrackLangEnvVariant}%
   \IfTrackedDialect{\@tracklang@dialect}%
   {%
      \let#2\@tracklang@dialect
   }%
   {%
      \edef\@tracklang@lang{\TrackLangGetKnownLangFromIso\@TrackLangEnvLang}%
      \edef\@tracklang@defscript{\TrackLangGetDefaultScript\@tracklang@lang}%
      \edef\@tracklang@dialects{\TrackedDialectsFromLanguage\@tracklang@lang}%
      \@tracklang@for\@tracklang@dialect:=\@tracklang@dialects\do{%
        \edef\@tracklang@tmp{%
          \TrackedIsoCodeFromLanguage{3166-1}{\@tracklang@dialect}}%
        \ifx\@tracklang@tmp\@TrackLangEnvTerritory
          \edef\@tracklang@tmp{%
            \GetTrackedDialectSubLang{\@tracklang@dialect}}%
          \ifx\@tracklang@tmp\@TrackLangEnvSubLang
            \edef\@tracklang@tmp{%
              \GetTrackedDialectVariant{\@tracklang@dialect}}%
            \ifx\@tracklang@tmp\@TrackLangEnvVariant
              \edef\@tracklang@tmp{%
                \GetTrackedDialectScript{\@tracklang@dialect}}%
              \ifx\@tracklang@tmp\@TrackLangEnvScript
                \let#2\@tracklang@dialect
              \else
                \ifx\@TrackLangEnvScript\empty
                  \ifx\@tracklang@tmp\@tracklang@defscript
                    \let#2\@tracklang@dialect
                  \fi
                \fi
              \fi
            \fi
          \fi
        \fi
      }%
   }%
}
\def\TrackLangFromEnv{%
 \def\TrackLangEnvLang{}%
 \def\TrackLangEnvTerritory{}%
 \def\TrackLangEnvCodeSet{}%
 \def\TrackLangEnvModifier{}%
  \ifx\TrackLangEnv\undefined
    \TrackLangQueryEnv
  \fi
  \ifx\TrackLangEnv\empty
     \@tracklang@warn{\string\TrackLangFromEnv\space
     non-operational as \string\TrackLangEnv\space is empty}%
  \else
    \ifx\TrackLangEnv\undefined
       \@tracklang@warn{\string\TrackLangFromEnv\space
       non-operational as \string\TrackLangEnv\space hasn't been
       defined}%
    \else
       \@tracklang@parse@track@locale{\TrackLangEnv}%
       \let\TrackLangEnvLang\@TrackLangEnvLang
       \let\TrackLangEnvTerritory\@TrackLangEnvTerritory
       \let\TrackLangEnvCodeSet\@TrackLangEnvCodeSet
       \let\TrackLangEnvModifier\@TrackLangEnvModifier
    \fi
  \fi
}
\def\TrackLocale#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \@tracklang@parse@track@locale{#1}%
  }%
  {%
    \@tracklang@nameuse{@tracklang@add@#1}%
  }%
}
\def\@tracklang@parse@track@locale#1{%
  \@tracklang@parse@locale{#1}%
  \@tracklang@track@locale
}
\def\@tracklang@track@locale{%
  \TrackLangIfKnownLangFromIso{\@TrackLangEnvLang}
  {%
    \edef\@tracklang@lang{\TrackLangGetKnownLangFromIso\@TrackLangEnvLang}%
    \let\@tracklang@dialect\@TrackLangEnvLang
    \ifx\@TrackLangEnvSubLang\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvSubLang}%
    \fi
    \ifx\@TrackLangEnvScript\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvScript}%
    \fi
    \ifx\@TrackLangEnvTerritory\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvTerritory}%
    \fi
    \ifx\@TrackLangEnvModifier\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvModifier}%
    \fi
    \ifx\@TrackLangEnvVariant\empty
    \else
      \edef\@tracklang@dialect{\@tracklang@dialect-\@TrackLangEnvVariant}%
    \fi
    \@tracklang@ifundef{@tracklang@add@\@tracklang@dialect}%
    {%
       \edef\@tracklang@dialect{%
         \@TrackLangEnvLang
         \@TrackLangEnvSubLang
         \@TrackLangEnvScript
         \@TrackLangEnvTerritory
         \@TrackLangEnvModifier
         \@TrackLangEnvVariant}%
       \AddTrackedDialect{\@tracklang@dialect}{\@tracklang@lang}%
       \AddTrackedLanguageIsoCodes{\@tracklang@lang}%
       \ifx\@TrackLangEnvFirstSubLang\empty
       \else
         \expandafter\AddTrackedIsoLanguage
           \expandafter\ThreeLetterExtIsoLanguageCode
           \expandafter{\@TrackLangEnvFirstSubLang}%
           {\@tracklang@dialect}%
       \fi
    }%
    {%
      \csname @tracklang@add@\@tracklang@dialect\endcsname
    }%
  }%
  {%
    \@tracklang@warn{Unknown language code `\@TrackLangEnvLang'}%
    \edef\@tracklang@dialect{%
      \@TrackLangEnvLang
      \@TrackLangEnvSubLang
      \@TrackLangEnvScript
      \@TrackLangEnvTerritory
      \@TrackLangEnvModifier
      \@TrackLangEnvVariant}%
    \AddTrackedDialect{\@tracklang@dialect}{\@TrackLangEnvLang}%
    \expandafter\@tracklang@hasthirdchar
       \@TrackLangEnvLang\relax\relax\relax\@end@tracklang@hasthirdchar
     {%
       \AddTrackedIsoLanguage{639-2}{\@TrackLangEnvLang}{\@tracklang@lang}%
     }%
     {%
         \AddTrackedIsoLanguage{639-1}{\@TrackLangEnvLang}{\@tracklang@lang}%
     }%
  }%
  \ifx\@TrackLangEnvTerritory\empty
  \else
    \AddTrackedIsoLanguage{3166-1}{\@TrackLangEnvTerritory}%
     {\@tracklang@dialect}%
  \fi
  \ifx\@TrackLangEnvModifier\empty
  \else
    \SetTrackedDialectModifier{\@tracklang@dialect}{\@TrackLangEnvModifier}%
  \fi
  \ifx\@TrackLangEnvVariant\empty
  \else
    \SetTrackedDialectVariant{\@tracklang@dialect}{\@TrackLangEnvVariant}%
  \fi
  \ifx\@TrackLangEnvScript\empty
  \else
    \SetTrackedDialectScript{\@tracklang@dialect}{\@TrackLangEnvScript}%
  \fi
  \ifx\@TrackLangEnvSubLang\empty
  \else
    \SetTrackedDialectSubLang{\@tracklang@dialect}{\@TrackLangEnvSubLang}%
  \fi
  \ifx\@TrackLangEnvAdditional\empty
  \else
    \SetTrackedDialectAdditional{\@tracklang@dialect}{\@TrackLangEnvAdditional}%
  \fi
}
\ifx\@tracklang@declareoption\undefined
  \def\@tracklang@declareoption#1{}
\fi
\def\TrackLangDeclareLanguageOption#1#2#3#4#5#6#7{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \TrackLangNewLanguage{#1}{#2}{#3}{#4}{#5}{#6}{#7}%
    \@tracklang@namedef{@tracklang@add@#1}{%
      \AddTrackedLanguage{#1}%
      \AddTrackedLanguageIsoCodes{#1}%
      \AddTrackedCountryIsoCode{#1}%
    }%
    \@tracklang@declareoption{#1}%
  }%
  {%
    \@tracklang@err{language option `#1' has already been defined}{}%
  }%
}
\TrackLangDeclareLanguageOption{abkhaz}{ab}{abk}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{afar}{aa}{aar}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{afrikaans}{af}{afr}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{akan}{ak}{aka}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{albanian}{sq}{sqi}{alb}{}{}{Latn}
\TrackLangDeclareLanguageOption{amharic}{am}{amh}{}{}{ET}{Ethi}
\TrackLangDeclareLanguageOption{anglosaxon}{}{ang}{}{}{}{Runr}
\TrackLangDeclareLanguageOption{apache}{}{apa}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{arabic}{ar}{ara}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{aragonese}{an}{arg}{}{}{ES}{Latn}
\TrackLangDeclareLanguageOption{armenian}{hy}{hye}{arm}{}{}{Armn}
\TrackLangDeclareLanguageOption{assamese}{as}{asm}{}{}{}{Beng}
\TrackLangDeclareLanguageOption{asturian}{}{ast}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{avaric}{av}{ava}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{avestan}{ae}{ave}{}{}{}{Avst}
\TrackLangDeclareLanguageOption{aymara}{ay}{aym}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{azerbaijani}{az}{aze}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{bahasai}{id}{ind}{}{}{IN}{Latn}
\TrackLangDeclareLanguageOption{bahasam}{ms}{msa}{may}{}{MY}{Latn}
\TrackLangDeclareLanguageOption{bambara}{bm}{bam}{}{}{ML}{Latn}
\TrackLangDeclareLanguageOption{bashkir}{ba}{bak}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{basque}{eu}{eus}{baq}{}{}{Latn}
\TrackLangDeclareLanguageOption{belarusian}{be}{bel}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{bengali}{bn}{ben}{}{}{}{Beng}
\TrackLangDeclareLanguageOption{berber}{}{ber}{}{}{}{}
\TrackLangDeclareLanguageOption{bihari}{bh}{bih}{}{}{}{}
\TrackLangDeclareLanguageOption{bislama}{bi}{bis}{}{}{VU}{Latn}
\TrackLangDeclareLanguageOption{bokmal}{nb}{nob}{}{}{NO}{Latn}
\TrackLangDeclareLanguageOption{bosnian}{bs}{bos}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{breton}{br}{bre}{}{}{FR}{Latn}
\TrackLangDeclareLanguageOption{bulgarian}{bg}{bul}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{burmese}{my}{mya}{bur}{}{}{Mymr}
\TrackLangDeclareLanguageOption{catalan}{ca}{cat}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chamorro}{ch}{cha}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chechen}{ce}{che}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{chichewa}{ny}{nya}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{chinese}{zh}{zho}{chi}{}{}{Hans}
\TrackLangDeclareLanguageOption{churchslavonic}{cu}{chu}{}{}{}{Glag}
\TrackLangDeclareLanguageOption{chuvash}{cv}{chv}{}{}{RU}{Cyrl}
\TrackLangDeclareLanguageOption{coptic}{}{cop}{}{}{}{Copt}
\TrackLangDeclareLanguageOption{cornish}{kw}{cor}{}{}{GB}{Latn}
\TrackLangDeclareLanguageOption{corsican}{co}{cos}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{cree}{cr}{cre}{}{}{}{Cans}
\TrackLangDeclareLanguageOption{croatian}{hr}{hrv}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{czech}{cs}{ces}{cze}{}{}{Latn}
\TrackLangDeclareLanguageOption{danish}{da}{dan}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{divehi}{dv}{div}{}{}{MV}{Thaa}
\TrackLangDeclareLanguageOption{dutch}{nl}{nld}{dut}{}{}{Latn}
\TrackLangDeclareLanguageOption{dzongkha}{dz}{dzo}{}{}{BT}{Tibt}
\TrackLangDeclareLanguageOption{easternpunjabi}{pa}{pan}{}{}{IN}{Guru}
\TrackLangDeclareLanguageOption{english}{en}{eng}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{esperanto}{eo}{epo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{estonian}{et}{est}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ewe}{ee}{ewe}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{faroese}{fo}{fao}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{farsi}{fa}{fas}{per}{}{}{Arab}
\TrackLangDeclareLanguageOption{fijian}{fj}{fij}{}{}{FJ}{Latn}
\TrackLangDeclareLanguageOption{finnish}{fi}{fin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{french}{fr}{fra}{fre}{}{}{Latn}
\TrackLangDeclareLanguageOption{friulan}{}{fur}{}{}{IT}{Latn}
\TrackLangDeclareLanguageOption{fula}{ff}{ful}{}{}{}{}
\TrackLangDeclareLanguageOption{galician}{gl}{glg}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ganda}{lg}{lug}{}{}{UG}{Latn}
\TrackLangDeclareLanguageOption{georgian}{ka}{kat}{geo}{}{}{Geor}
\TrackLangDeclareLanguageOption{german}{de}{deu}{ger}{}{}{Latn}
\TrackLangDeclareLanguageOption{greek}{el}{ell}{gre}{}{}{Grek}
\TrackLangDeclareLanguageOption{guarani}{gn}{grn}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{gujarati}{gu}{guj}{}{}{}{Gujr}
\TrackLangDeclareLanguageOption{haitian}{ht}{hat}{}{}{HT}{Latn}
\TrackLangDeclareLanguageOption{hausa}{ha}{hau}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{hebrew}{he}{heb}{}{}{}{Hebr}
\TrackLangDeclareLanguageOption{herero}{hz}{her}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{hindi}{hi}{hin}{}{}{}{Deva}
\TrackLangDeclareLanguageOption{hirimotu}{ho}{hmo}{}{}{PG}{Latn}
\TrackLangDeclareLanguageOption{icelandic}{is}{isl}{ice}{}{IS}{Latn}
\TrackLangDeclareLanguageOption{ido}{io}{ido}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{igbo}{ig}{ibo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{interlingua}{ia}{ina}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{interlingue}{ie}{ile}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{inuktitut}{iu}{iku}{}{}{}{Cans}
\TrackLangDeclareLanguageOption{inupiaq}{ik}{ipk}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{irish}{ga}{gle}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{italian}{it}{ita}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{japanese}{ja}{jpn}{}{}{}{Hani}
\TrackLangDeclareLanguageOption{javanese}{jv}{jav}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kalaallisut}{kl}{kal}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kannada}{kn}{kan}{}{}{IN}{Knda}
\TrackLangDeclareLanguageOption{kanuri}{kr}{kau}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kashmiri}{ks}{kas}{}{}{IN}{}
\TrackLangDeclareLanguageOption{kazakh}{kk}{kaz}{}{}{}{}
\TrackLangDeclareLanguageOption{khmer}{km}{khm}{}{}{}{Khmr}
\TrackLangDeclareLanguageOption{kikuyu}{ki}{kik}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kinyarwanda}{rw}{kin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kirundi}{rn}{run}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{komi}{kv}{kom}{}{}{RU}{Cyrl}
\TrackLangDeclareLanguageOption{kongo}{kg}{kon}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{korean}{ko}{kor}{}{}{}{Hang}
\TrackLangDeclareLanguageOption{kurdish}{ku}{kur}{}{}{}{}
\TrackLangDeclareLanguageOption{kwanyama}{kj}{kua}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{kyrgyz}{ky}{kir}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{lao}{lo}{lao}{}{}{}{Laoo}
\TrackLangDeclareLanguageOption{latin}{la}{lat}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{latvian}{lv}{lav}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{limburgish}{li}{lim}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lingala}{ln}{lin}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lithuanian}{lt}{lit}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{lsorbian}{}{dsb}{}{}{DE}{Latn}
\TrackLangDeclareLanguageOption{lubakatanga}{lu}{lub}{}{}{CD}{Latn}
\TrackLangDeclareLanguageOption{luxembourgish}{lb}{ltz}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{macedonian}{mk}{mkd}{mac}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{magyar}{hu}{hun}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{malagasy}{mg}{mlg}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{malayalam}{ml}{mal}{}{}{IN}{Mlym}
\TrackLangDeclareLanguageOption{maltese}{mt}{mlt}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{manx}{gv}{glv}{}{}{IM}{Latn}
\TrackLangDeclareLanguageOption{maori}{mi}{mri}{mao}{}{NZ}{Latn}
\TrackLangDeclareLanguageOption{marathi}{mr}{mar}{}{}{IN}{Deva}
\TrackLangDeclareLanguageOption{marshallese}{mh}{mah}{}{}{MH}{Latn}
\TrackLangDeclareLanguageOption{mongolian}{mn}{mon}{}{}{}{Mong}
\TrackLangDeclareLanguageOption{nauruan}{na}{nau}{}{}{NR}{Latn}
\TrackLangDeclareLanguageOption{navajo}{nv}{nav}{}{}{US}{Latn}
\TrackLangDeclareLanguageOption{ndonga}{ng}{ndo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nepali}{ne}{nep}{}{}{}{Deva}
\TrackLangDeclareLanguageOption{nko}{}{nqo}{}{}{}{Nkoo}
\TrackLangDeclareLanguageOption{northernndebele}{nd}{nde}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nynorsk}{nn}{nno}{}{}{NO}{Latn}
\TrackLangDeclareLanguageOption{norsk}{no}{nor}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{northernsotho}{}{nso}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{nuosu}{ii}{iii}{}{}{CN}{Yiii}
\TrackLangDeclareLanguageOption{occitan}{oc}{oci}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{ojibwe}{oj}{oji}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{oromo}{om}{orm}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{oriya}{or}{ori}{}{}{}{Orya}
\TrackLangDeclareLanguageOption{ossetian}{os}{oss}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{pali}{pi}{pli}{}{}{}{Brah}
\TrackLangDeclareLanguageOption{pashto}{ps}{pus}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{piedmontese}{}{}{}{pms}{IT}{Latn}
\TrackLangDeclareLanguageOption{polish}{pl}{pol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{portuges}{pt}{por}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{quechua}{qu}{que}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{romanian}{ro}{ron}{rum}{}{}{Latn}
\TrackLangDeclareLanguageOption{romansh}{rm}{roh}{}{}{CH}{Latn}
\TrackLangDeclareLanguageOption{russian}{ru}{rus}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{samin}{se}{sme}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sanskrit}{sa}{san}{}{}{}{}
\TrackLangDeclareLanguageOption{samoan}{sm}{smo}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sango}{sg}{sag}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sardinian}{sc}{srd}{}{}{IT}{Latn}
\TrackLangDeclareLanguageOption{scottish}{gd}{gla}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{serbian}{sr}{srp}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{shona}{sn}{sna}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sindhi}{sd}{snd}{}{}{}{Sind}
\TrackLangDeclareLanguageOption{sinhalese}{si}{sin}{}{}{LK}{Sinh}
\TrackLangDeclareLanguageOption{slovak}{sk}{slk}{slo}{}{}{Latn}
\TrackLangDeclareLanguageOption{slovene}{sl}{slv}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{somali}{so}{som}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{southernndebele}{nr}{nbl}{}{}{ZA}{Latn}
\TrackLangDeclareLanguageOption{southernsotho}{st}{sot}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{spanish}{es}{spa}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{sudanese}{su}{sun}{}{}{}{Sund}
\TrackLangDeclareLanguageOption{swahili}{sw}{swa}{}{}{}{}
\TrackLangDeclareLanguageOption{swati}{ss}{ssw}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{swedish}{sv}{swe}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{syriac}{}{syr}{}{}{}{Syrc}
\TrackLangDeclareLanguageOption{tagalog}{tl}{tgl}{}{}{PH}{Latn}
\TrackLangDeclareLanguageOption{tahitian}{ty}{tah}{}{}{PF}{Latn}
\TrackLangDeclareLanguageOption{tai}{}{tai}{}{}{}{}
\TrackLangDeclareLanguageOption{tajik}{tg}{tgk}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{tamil}{ta}{tam}{}{}{}{Taml}
\TrackLangDeclareLanguageOption{tatar}{tt}{tat}{}{}{}{Cyrl}
\TrackLangDeclareLanguageOption{telugu}{te}{tel}{}{}{IN}{Telu}
\TrackLangDeclareLanguageOption{thai}{th}{tha}{}{}{TH}{Thai}
\TrackLangDeclareLanguageOption{tibetan}{bo}{bod}{tib}{}{}{Tibt}
\TrackLangDeclareLanguageOption{tigrinya}{ti}{tir}{}{}{}{Ethi}
\TrackLangDeclareLanguageOption{tonga}{to}{ton}{}{}{TO}{Latn}
\TrackLangDeclareLanguageOption{tsonga}{ts}{tso}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{tswana}{tn}{tsn}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{turkish}{tr}{tur}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{turkmen}{tk}{tuk}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{twi}{tw}{twi}{}{}{GH}{Latn}
\TrackLangDeclareLanguageOption{ukrainian}{uk}{ukr}{}{}{UA}{Cyrl}
\TrackLangDeclareLanguageOption{urdu}{ur}{urd}{}{}{}{Arab}
\TrackLangDeclareLanguageOption{usorbian}{}{hsb}{}{}{DE}{Latn}
\TrackLangDeclareLanguageOption{uyghur}{ug}{uig}{}{}{CN}{Arab}
\TrackLangDeclareLanguageOption{uzbek}{uz}{uzb}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{venda}{ve}{ven}{}{}{ZA}{Latn}
\TrackLangDeclareLanguageOption{vietnamese}{vi}{vie}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{volapuk}{vo}{vol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{walloon}{wa}{wln}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{welsh}{cy}{cym}{wel}{}{}{Latn}
\TrackLangDeclareLanguageOption{westernfrisian}{fy}{fry}{}{}{NL}{Latn}
\TrackLangDeclareLanguageOption{wolof}{wo}{wol}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{xhosa}{xh}{xho}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{yiddish}{yi}{yid}{}{}{}{Hebr}
\TrackLangDeclareLanguageOption{yoruba}{yo}{yor}{}{}{}{Latn}
\TrackLangDeclareLanguageOption{zhuang}{za}{zha}{}{}{CN}{Hani}
\TrackLangDeclareLanguageOption{zulu}{zu}{zul}{}{}{}{Latn}
\def\TrackLangDeclareDialectOption#1#2#3#4#5#6#7{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \ifx\relax#3\relax
     \ifx\relax#4\relax
      \ifx\relax#5\relax
        \@tracklang@namedef{@tracklang@add@#1}{%
          \AddTrackedDialect{#1}{#2}%
          \AddTrackedLanguageIsoCodes{#2}%
          \def\@tracklang@dialect{#1}%
        }%
      \else
        \@tracklang@namedef{@tracklang@add@#1}{%
          \AddTrackedDialect{#1}{#2}%
          \AddTrackedLanguageIsoCodes{#2}%
          \SetTrackedDialectVariant{#1}{#5}%
          \def\@tracklang@dialect{#1}%
        }%
      \fi
     \else
       \ifx\relax#5\relax
         \@tracklang@namedef{@tracklang@add@#1}{%
           \AddTrackedDialect{#1}{#2}%
           \AddTrackedLanguageIsoCodes{#2}%
           \SetTrackedDialectModifier{#1}{#4}%
           \def\@tracklang@dialect{#1}%
         }%
       \else
         \@tracklang@namedef{@tracklang@add@#1}{%
           \AddTrackedDialect{#1}{#2}%
           \AddTrackedLanguageIsoCodes{#2}%
           \SetTrackedDialectModifier{#1}{#4}%
           \SetTrackedDialectVariant{#1}{#5}%
           \def\@tracklang@dialect{#1}%
         }%
       \fi
     \fi
    \else
     \ifx\relax#4\relax
       \ifx\relax#5\relax
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \def\@tracklang@dialect{#1}%
          }%
       \else
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectVariant{#1}{#5}%
            \def\@tracklang@dialect{#1}%
          }%
       \fi
     \else
       \ifx\relax#5\relax
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectModifier{#1}{#4}%
            \def\@tracklang@dialect{#1}%
          }%
       \else
          \@tracklang@namedef{@tracklang@add@#1}{%
            \AddTrackedDialect{#1}{#2}%
            \AddTrackedLanguageIsoCodes{#2}%
            \AddTrackedIsoLanguage{3166-1}{#3}{#1}%
            \SetTrackedDialectModifier{#1}{#4}%
            \SetTrackedDialectVariant{#1}{#5}%
            \def\@tracklang@dialect{#1}%
          }%
       \fi
     \fi
    \fi
    \ifx\relax#6\relax
    \else
      \expandafter
       \let\expandafter\@tracklang@tmp\csname @tracklang@add@#1\endcsname
      \expandafter\def\csname @tracklang@add@#1\expandafter\endcsname
        \expandafter{\@tracklang@tmp\SetTrackedDialectLabelMap{#1}{#6}}%
    \fi
    \ifx\relax#7\relax
    \else
      \expandafter
       \let\expandafter\@tracklang@tmp\csname @tracklang@add@#1\endcsname
      \expandafter\def\csname @tracklang@add@#1\expandafter\endcsname
        \expandafter{\@tracklang@tmp\SetTrackedDialectScript{#1}{#7}}%
    \fi
    \@tracklang@declareoption{#1}%
  }%
  {%
    \@tracklang@err{dialect option `#1' has already been defined}{}%
  }%
}
\TrackLangDeclareDialectOption{acadian}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{american}{english}{US}{}{}{}{}
\TrackLangDeclareDialectOption{australian}{english}{AU}{}{}{}{}
\TrackLangDeclareDialectOption{austrian}{german}{AT}{}{}{}{}
\TrackLangDeclareDialectOption{naustrian}{german}{AT}{new}{1996}{}{}
\TrackLangDeclareDialectOption{bahasa}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{brazil}{portuges}{BR}{}{}{}{}
\TrackLangDeclareDialectOption{brazilian}{portuges}{BR}{}{}{}{}
\TrackLangDeclareDialectOption{british}{english}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{canadian}{english}{CA}{}{}{}{}
\TrackLangDeclareDialectOption{canadien}{french}{CA}{}{}{}{}
\TrackLangDeclareDialectOption{croatia}{croatian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{istriacountycroatian}{croatian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{istriacountyitalian}{italian}{HR}{}{}{}{}
\TrackLangDeclareDialectOption{netherlands}{dutch}{NL}{}{}{}{}
\TrackLangDeclareDialectOption{persian}{farsi}{}{}{}{}{}
\TrackLangDeclareDialectOption{flemish}{dutch}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{francais}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{frenchb}{french}{}{}{}{}{}
\TrackLangDeclareDialectOption{france}{french}{FR}{}{}{}{}
\TrackLangDeclareDialectOption{belgique}{french}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{belgiangerman}{german}{BE}{}{}{}{}
\TrackLangDeclareDialectOption{nbelgiangerman}{german}{BE}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{friulian}{friulan}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{friulano}{friulan}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{galicien}{galician}{}{}{}{}{}
\TrackLangDeclareDialectOption{deutsch}{german}{}{}{}{}{}
\TrackLangDeclareDialectOption{ngerman}{german}{}{new}{1996}{}{}
\TrackLangDeclareDialectOption{ngermanb}{german}{}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{germanb}{german}{}{}{}{}{}
\TrackLangDeclareDialectOption{ngermanDE}{german}{DE}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{germanDE}{german}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{hungarian}{magyar}{HU}{}{}{}{}
\TrackLangDeclareDialectOption{indon}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{indonesian}{bahasai}{IN}{}{}{}{}
\TrackLangDeclareDialectOption{gaeilge}{irish}{}{}{}{}{}
\TrackLangDeclareDialectOption{IEirish}{irish}{IE}{}{}{}{}
\TrackLangDeclareDialectOption{GBirish}{irish}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{IEenglish}{english}{IE}{}{}{british}{}
\TrackLangDeclareDialectOption{italy}{italian}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{vatican}{italian}{VA}{}{}{}{}
\TrackLangDeclareDialectOption{sanmarino}{italian}{SM}{}{}{}{}
\TrackLangDeclareDialectOption{sloveneistriaitalian}{italian}{SI}{}{}{}{}
\TrackLangDeclareDialectOption{jerseyenglish}{english}{JE}{}{}{british}{}
\TrackLangDeclareDialectOption{jerseyfrench}{french}{JE}{}{}{}{}
\TrackLangDeclareDialectOption{guernseyenglish}{english}{GG}{}{}{british}{}
\TrackLangDeclareDialectOption{guernseyfrench}{french}{GG}{}{}{}{}
\TrackLangDeclareDialectOption{latein}{latin}{}{}{}{}{}
\TrackLangDeclareDialectOption{lowersorbian}{lsorbian}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{malay}{bahasam}{MY}{}{}{}{}
\TrackLangDeclareDialectOption{meyalu}{bahasam}{MY}{}{}{}{}
\TrackLangDeclareDialectOption{maltamaltese}{maltese}{MT}{}{}{}{}
\TrackLangDeclareDialectOption{maltaenglish}{english}{MT}{}{}{british}{}
\TrackLangDeclareDialectOption{newzealand}{english}{NZ}{}{}{}{}
\TrackLangDeclareDialectOption{isleofmanenglish}{english}{IM}{}{}{british}{}
\TrackLangDeclareDialectOption{norwegian}{norsk}{NO}{}{}{}{}
\TrackLangDeclareDialectOption{piemonteis}{piedmontese}{IT}{}{}{}{}
\TrackLangDeclareDialectOption{polutonikogreek}{greek}{}{polyton}{}{}{}
\TrackLangDeclareDialectOption{polutoniko}{greek}{}{polyton}{}{}{}
\TrackLangDeclareDialectOption{portuguese}{portuges}{}{}{}{}{}
\TrackLangDeclareDialectOption{portugal}{portuges}{PT}{}{}{}{}
\TrackLangDeclareDialectOption{romansch}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{rumantsch}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{romanche}{romansh}{}{}{}{}{}
\TrackLangDeclareDialectOption{russianb}{russian}{}{}{}{}{}
\TrackLangDeclareDialectOption{gaelic}{scottish}{}{}{}{}{}
\TrackLangDeclareDialectOption{GBscottish}{scottish}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{serbianc}{serbian}{}{}{}{}{Cyrl}
\TrackLangDeclareDialectOption{serbianl}{serbian}{}{}{}{}{Latn}
\TrackLangDeclareDialectOption{slovenian}{slovene}{}{}{}{}{}
\TrackLangDeclareDialectOption{slovenia}{slovene}{SI}{}{}{slovenian}{}
\TrackLangDeclareDialectOption{sloveneistriaslovenian}{slovene}{SI}{}{}{slovenian}{}
\TrackLangDeclareDialectOption{spainspanish}{spanish}{ES}{}{}{}{}
\TrackLangDeclareDialectOption{argentinespanish}{spanish}{AR}{}{}{}{}
\TrackLangDeclareDialectOption{bolivianspanish}{spanish}{BO}{}{}{}{}
\TrackLangDeclareDialectOption{chilianspanish}{spanish}{CL}{}{}{}{}
\TrackLangDeclareDialectOption{columbianspanish}{spanish}{CO}{}{}{}{}
\TrackLangDeclareDialectOption{costaricanspanish}{spanish}{CR}{}{}{}{}
\TrackLangDeclareDialectOption{cubanspanish}{spanish}{CU}{}{}{}{}
\TrackLangDeclareDialectOption{dominicanspanish}{spanish}{DO}{}{}{}{}
\TrackLangDeclareDialectOption{ecudorianspanish}{spanish}{EC}{}{}{}{}
\TrackLangDeclareDialectOption{elsalvadorspanish}{spanish}{SV}{}{}{}{}
\TrackLangDeclareDialectOption{guatemalanspanish}{spanish}{GT}{}{}{}{}
\TrackLangDeclareDialectOption{honduranspanish}{spanish}{HN}{}{}{}{}
\TrackLangDeclareDialectOption{mexicanspanish}{spanish}{MX}{}{}{}{}
\TrackLangDeclareDialectOption{nicaraguanspanish}{spanish}{NI}{}{}{}{}
\TrackLangDeclareDialectOption{panamaspanish}{spanish}{PA}{}{}{}{}
\TrackLangDeclareDialectOption{paraguayspanish}{spanish}{PY}{}{}{}{}
\TrackLangDeclareDialectOption{peruvianspanish}{spanish}{PE}{}{}{}{}
\TrackLangDeclareDialectOption{puertoricospanish}{spanish}{PR}{}{}{}{}
\TrackLangDeclareDialectOption{uruguayspanish}{spanish}{UY}{}{}{}{}
\TrackLangDeclareDialectOption{venezuelanspanish}{spanish}{VE}{}{}{}{}
\TrackLangDeclareDialectOption{swissgerman}{german}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{nswissgerman}{german}{CH}{new}{1996}{ngerman}{}
\TrackLangDeclareDialectOption{swissfrench}{french}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{swissitalian}{italian}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{swissromansh}{romansh}{CH}{}{}{}{}
\TrackLangDeclareDialectOption{UKenglish}{english}{GB}{}{}{}{}
\TrackLangDeclareDialectOption{ukraineb}{ukrainian}{UA}{}{}{}{}
\TrackLangDeclareDialectOption{ukraine}{ukrainian}{UA}{}{}{}{}
\TrackLangDeclareDialectOption{uppersorbian}{usorbian}{DE}{}{}{}{}
\TrackLangDeclareDialectOption{USenglish}{english}{US}{}{}{}{}
\TrackLangDeclareDialectOption{valencian}{catalan}{}{}{}{}{}
\TrackLangDeclareDialectOption{valencien}{catalan}{}{}{}{}{}
\TrackLangDeclareDialectOption{cymraeg}{welsh}{}{}{}{}{}
\TrackLangDeclareDialectOption{GBwelsh}{welsh}{GB}{}{}{}{}
\def\LetTrackLangSynonym#1#2{%
  \expandafter\let\csname @tracklang@add@#1\expandafter\endcsname
    \csname @tracklang@add@#2\endcsname
}
\def\LetTrackLangOption#1#2{%
  \LetTrackLangSynonym{#1}{#2}%
  \@tracklang@declareoption{#1}%
}
\LetTrackLangOption{en-US}{american}
\LetTrackLangOption{en-GB}{british}
\LetTrackLangOption{en-AU}{australian}
\LetTrackLangOption{en-NZ}{newzealand}
\LetTrackLangOption{en-CA}{canadian}
\LetTrackLangOption{fr-CA}{canadien}
\LetTrackLangOption{fr-BE}{belgique}
\LetTrackLangOption{pt-BR}{brazilian}
\LetTrackLangOption{it-HR}{istriacountyitalian}
\LetTrackLangOption{nl-BE}{flemish}
\LetTrackLangOption{fr-FR}{france}
\LetTrackLangOption{de-DE}{germanDE}
\LetTrackLangOption{de-BE}{belgiangerman}
\LetTrackLangOption{en-GG}{guernseyenglish}
\LetTrackLangOption{fr-GG}{guernseyfrench}
\LetTrackLangOption{it-IT}{italy}
\LetTrackLangOption{mt-MT}{maltamaltese}
\LetTrackLangOption{en-MT}{maltaenglish}
\LetTrackLangOption{en-IM}{isleofmanenglish}
\LetTrackLangOption{en-JE}{jerseyenglish}
\LetTrackLangOption{fr-JE}{jerseyfrench}
\LetTrackLangOption{nl-NL}{netherlands}
\LetTrackLangOption{pt-PT}{portugal}
\LetTrackLangOption{it-SM}{sanmarino}
\LetTrackLangOption{sl-SI}{slovenia}
\LetTrackLangOption{it-SI}{sloveneistriaitalian}
\LetTrackLangOption{es-ES}{spainspanish}
\LetTrackLangOption{es-AR}{argentinespanish}
\LetTrackLangOption{es-BO}{bolivianspanish}
\LetTrackLangOption{es-CL}{chilianspanish}
\LetTrackLangOption{es-CO}{columbianspanish}
\LetTrackLangOption{es-CR}{costaricanspanish}
\LetTrackLangOption{es-CU}{cubanspanish}
\LetTrackLangOption{es-DO}{dominicanspanish}
\LetTrackLangOption{es-EC}{ecudorianspanish}
\LetTrackLangOption{es-SV}{elsalvadorspanish}
\LetTrackLangOption{es-GT}{guatemalanspanish}
\LetTrackLangOption{es-HN}{honduranspanish}
\LetTrackLangOption{es-MX}{mexicanspanish}
\LetTrackLangOption{es-NI}{nicaraguanspanish}
\LetTrackLangOption{es-PA}{panamaspanish}
\LetTrackLangOption{es-PY}{paraguayspanish}
\LetTrackLangOption{es-PE}{peruvianspanish}
\LetTrackLangOption{es-PR}{puertoricospanish}
\LetTrackLangOption{es-UY}{uruguayspanish}
\LetTrackLangOption{es-VE}{venezuelanspanish}
\LetTrackLangOption{de-CH}{swissgerman}
\LetTrackLangOption{fr-CH}{swissfrench}
\LetTrackLangOption{it-CH}{swissitalian}
\LetTrackLangOption{rm-CH}{swissromansh}
\LetTrackLangOption{it-VA}{vatican}
\LetTrackLangOption{ga-IE}{IEirish}
\LetTrackLangOption{ga-GB}{GBirish}
\LetTrackLangOption{en-IE}{IEenglish}
\LetTrackLangOption{de-AT-1996}{naustrian}
\LetTrackLangOption{de-AT}{austrian}
\LetTrackLangOption{id-IN}{bahasa}
\LetTrackLangOption{ms-MY}{malay}
\LetTrackLangOption{hr-HR}{croatia}
\LetTrackLangOption{de-DE-1996}{ngermanDE}
\LetTrackLangOption{de-CH-1996}{nswissgerman}
\LetTrackLangOption{hu-HU}{hungarian}
\LetTrackLangOption{gd-GB}{GBscottish}
\LetTrackLangOption{cy-GB}{GBwelsh}
\long\def\IfTrackedLanguage#1#2#3{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
    #3%
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}%
      \@tracklang@languages
    {%
      #2%
    }%
    {%
      #3%
    }%
  \fi
}
\long\def\IfTrackedDialect#1#2#3{%
  \@tracklang@ifundef{@tracklang@fromdialect@#1}{#3}{#2}%
}
\long\def\IfTrackedIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}{#4}{#3}%
}
\long\def\IfTrackedLanguageHasIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isofromlang@#2}{#4}{#3}%
}
\long\def\ForEachTrackedLanguage#1#2{%
  \@tracklang@for#1:=\@tracklang@languages\do{#2}%
}
\long\def\ForEachTrackedDialect#1#2{%
  \@tracklang@for#1:=\@tracklang@dialects\do{#2}%
}
\long\def\AnyTrackedLanguages#1#2{%
  \ifx\@tracklang@languages\empty
    #2%
  \else
    #1%
  \fi
}
\long\def\IfTrackedLanguageFileExists#1#2#3#4#5{%
   \def\CurrentTrackedTag{}%
   \SetCurrentTrackedDialect{#1}%
   \IfTrackedDialect{#1}%
   {%
     \edef\CurrentTrackedTag{#1}%
     \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
     {#4}%
     {%
       \IfTrackedLanguageHasIsoCode
         {639-1}{\CurrentTrackedLanguage}
       {%
          \edef\CurrentTrackedIsoCode{%
             \TrackedIsoCodeFromLanguage
               {639-1}{\CurrentTrackedLanguage}}%
          \ifx\CurrentTrackedRegion\empty
            \let\CurrentTrackedTag\CurrentTrackedIsoCode
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
                {639-2}{\CurrentTrackedLanguage}
              {%
                 \edef\CurrentTrackedIsoCode{%
                    \TrackedIsoCodeFromLanguage
                      {639-2}{\CurrentTrackedLanguage}}%
                 \let\CurrentTrackedTag\CurrentTrackedIsoCode
                 \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                 {#4}%
                 {%
                   \let\CurrentTrackedTag\CurrentTrackedLanguage
                   \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                 }%
              }%
              {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            }%
          \else
            \edef\CurrentTrackedTag{%
              \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
              {639-2}{\CurrentTrackedLanguage}
              {%
                \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                \edef\CurrentTrackedIsoCode{%
                  \TrackedIsoCodeFromLanguage
                  {639-2}{\CurrentTrackedLanguage}}%
                \edef\CurrentTrackedTag{%
                  \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\org@currenttrackedisocode
                  \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                  \let\CurrentTrackedIsoCode\CurrentTrackedTag
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}
                  {%
                    \let\CurrentTrackedIsoCode\org@currenttrackedisocode
                    \let\CurrentTrackedTag\CurrentTrackedIsoCode
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                    {#4}%
                    {%
                      \let\CurrentTrackedTag\CurrentTrackedRegion
                      \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                      {#4}%
                      {%
                        \let\CurrentTrackedTag\CurrentTrackedLanguage
                        \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                      }%
                    }%
                  }%
                }%
              }%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            }%
          \fi
       }%
       {%
         \IfTrackedLanguageHasIsoCode
           {639-2}{\CurrentTrackedLanguage}
         {%
            \edef\CurrentTrackedIsoCode{%
               \TrackedIsoCodeFromLanguage
               {639-2}{\CurrentTrackedLanguage}}%
         }%
         {%
           \IfTrackedLanguageHasIsoCode
             {639-3}{\CurrentTrackedLanguage}
           {%
              \edef\CurrentTrackedIsoCode{%
                 \TrackedIsoCodeFromLanguage
                 {639-3}{\CurrentTrackedLanguage}}%
           }%
           {%
              \let\CurrentTrackedIsoCode\empty
           }%
         }%
         \ifx\CurrentTrackedIsoCode\empty
           \ifx\CurrentTrackedRegion\empty
             \let\CurrentTrackedTag\CurrentTrackedLanguage
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
           \else
             \let\CurrentTrackedTag\CurrentTrackedRegion
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
             {#4}%
             {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
             }%
           \fi
         \else
            \ifx\CurrentTrackedRegion\empty
              \let\CurrentTrackedTag\CurrentTrackedIsoCode
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedLanguage
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            \else
              \edef\CurrentTrackedTag{%
                \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            \fi
         \fi
       }%
     }%
   }%
   {#5}% unknown dialect
}
\ifx\ProvidesFile\undefined
  \long\def\TrackLangProvidesResource#1#2{%
    \ifx\TrackLangRequireDialectPrefix\undefined
      \@tracklang@err{Resources files using
        \string\TrackLangProvidesResource\space
        must be loaded with \string\TrackLangRequireDialect}%
    \fi
    \ifx#2[\relax
      \def\@tracklang@next{%
        \@tracklang@providesresource{\TrackLangRequireDialectPrefix-#1.ldf}#2%
      }
    \else
      \expandafter\xdef\csname ver@\TrackLangRequireDialectPrefix
        -#1.ldf\endcsname{}%
      {%
        \newlinechar=`\^^J
        \def\MessageBreak{^^J}%
        \message{^^JFile: \TrackLangRequireDialectPrefix-#1.ldf^^J}%
      }%
      \long\def\@tracklang@next{#2}%
    \fi
    \@tracklang@next
  }
  \def\@tracklang@providesresource#1[#2]{%
    \expandafter\xdef\csname ver@#1\endcsname{#2}%
     {%
       \newlinechar=`\^^J
       \def\MessageBreak{^^J}%
       \message{^^JFile: #1 #2^^J}%
     }%
  }
\else
  \def\TrackLangProvidesResource#1{%
    \ifx\TrackLangRequireDialectPrefix\undefined
      \@tracklang@err{Resources files using
        \string\TrackLangProvidesResource\space
        must be loaded with \string\TrackLangRequireDialect}%
    \fi
    \ProvidesFile{\TrackLangRequireDialectPrefix-#1.ldf}%
  }
\fi
\def\TrackLangAddToHook{\noop@TrackLangAddToHook}
\def\noop@TrackLangAddToHook#1#2{%
  \@tracklang@err{\string\TrackLangAddToHook\space
  only permitted within resource files}
}
\def\@TrackLangAddToHook#1#2{%
  \@tracklang@ifundef{#2\CurrentTrackedDialect}%
  {%
    \IfTrackedDialectHasMapping{\CurrentTrackedDialect}%
    {%
      \edef\@tracklang@tmp{%
        \csname @tracklang@dialectmap@tohook@\CurrentTrackedDialect\endcsname}%
      \@tracklang@ifundef{#2\@tracklang@tmp}%
      {%
        \@tracklang@ifundef{#2\CurrentTrackedLanguage}%
        {%
          #1%
        }%
        {%
          \@tracklang@addtohook{#2}{\CurrentTrackedLanguage}{#1}%
        }%
      }%
      {%
        \@tracklang@addtohook{#2}{\@tracklang@tmp}{#1}%
      }%
    }%
    {%
      \@tracklang@ifundef{#2\CurrentTrackedLanguage}%
      {%
      }%
      {%
        \@tracklang@addtohook{#2}{\CurrentTrackedLanguage}{#1}%
      }%
    }%
  }%
  {%
     \@tracklang@addtohook{#2}{\CurrentTrackedDialect}{#1}%
  }%
  #1%
}
\def\@tracklang@addtohook#1#2#3{%
 \expandafter\let\expandafter\@tracklang@hook\csname #1#2\endcsname
 \expandafter
  \gdef\csname#1#2\expandafter\endcsname\expandafter{\@tracklang@hook#3}%
}
\def\TrackLangAddToCaptions#1{\TrackLangAddToHook{#1}{captions}}
\def\SetTrackedDialectLabelMap#1#2{%
  \@tracklang@enamedef{@tracklang@dialectmap@tohook@#1}{#2}%
  \@tracklang@enamedef{@tracklang@dialectmap@fromhook@#2}{#1}%
}
\def\IfTrackedDialectHasMapping#1#2#3{%
  \@tracklang@ifundef{@tracklang@dialectmap@tohook@#1}{#3}{#2}%
}
\def\IfHookHasMappingFromTrackedDialect#1#2#3{%
  \@tracklang@ifundef{@tracklang@dialectmap@fromhook@#1}{#3}{#2}%
}
\def\GetTrackedDialectToMapping#1{%
  \@tracklang@ifundef{@tracklang@dialectmap@tohook@#1}{#1}%
  {\csname @tracklang@dialectmap@tohook@#1\endcsname}%
}
\def\GetTrackedDialectFromMapping#1{%
  \@tracklang@ifundef{@tracklang@dialectmap@fromhook@#1}{#1}%
  {\csname @tracklang@dialectmap@fromhook@#1\endcsname}%
}
\def\TrackLangRequireResource{\noop@TrackLangRequireResource}
\def\noop@TrackLangRequireResource#1{%
  \@tracklang@err{\string\TrackLangRequireResource\space
  only permitted within resource files}
}
\def\@TrackLangRequireResource#1{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
    }%
    {%
      \@tracklang@warn{No `\TrackLangRequireDialectPrefix' support for
      language/region `#1'\MessageBreak
      (resource file `\TrackLangRequireDialectPrefix-#1.ldf' not found)}%
    }%
  }%
  {}%
}
\def\TrackLangRequireResourceOrDo{%
  \noop@TrackLangRequireResourceOrDo
}
\def\noop@TrackLangRequireResourceOrDo#1#2#3{%
  \@tracklang@err{\string\TrackLangRequireResourceOrDo\space
  only permitted within resource files}
}
\def\@TrackLangRequireResourceOrDo#1#2#3{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
      #2%
    }%
    {%
      \@tracklang@warn{No `\TrackLangRequireDialectPrefix' support for
      language/region `#1'\MessageBreak
      (resource file `\TrackLangRequireDialectPrefix-#1.ldf' not found)}%
    }%
  }%
  {#3}%
}
\def\TrackLangRequestResource{\noop@TrackLangRequestResource}
\def\noop@TrackLangRequestResource#1#2{%
  \@tracklang@err{\string\TrackLangRequestResource\space
  only permitted within resource files}
}
\def\@TrackLangRequestResource#1#2{%
  \@tracklang@ifundef{ver@\TrackLangRequireDialectPrefix-#1.ldf}%
  {%
    \@tracklang@IfFileExists{\TrackLangRequireDialectPrefix-#1.ldf}%
    {%
      \input \TrackLangRequireDialectPrefix-#1.ldf
    }%
    {#2}%
  }%
  {}%
}
\def\TrackLangRequireDialect{\@TrackLangRequireDialect}
\def\noop@TrackLangRequireDialect#1{%
  \ifx[#1\relax
    \def\@tracklang@next{\@noop@TrackLangRequireDialect[}%
  \else
    \def\@tracklang@next{\@noop@TrackLangRequireDialect[]{#1}}%
  \fi
  \@tracklang@next
}
\def\@noop@TrackLangRequireDialect[#1]#2#3{%
  \@tracklang@err{\string\TrackLangRequireDialect\space
  only permitted within resource files}
}
\def\@TrackLangRequireDialect#1{%
  \ifx[#1\relax
    \def\@tracklang@next{\@@TrackLangRequireDialect[}%
  \else
    \def\@tracklang@next{%
      \@@TrackLangRequireDialect
        [\TrackLangRequireResource{\CurrentTrackedTag}]{#1}}%
  \fi
  \@tracklang@next
}
\def\@@TrackLangRequireDialect[#1]#2#3{%
   \def\TrackLangRequireDialectPrefix{#2}%
   \IfTrackedLanguageFileExists{#3}%
   {#2-}% prefix
   {.ldf}% suffix
   {%
     \let\TrackLangRequireResource\@TrackLangRequireResource
     \let\TrackLangRequireResourceOrDo\@TrackLangRequireResourceOrDo
     \let\TrackLangRequestResource\@TrackLangRequestResource
     \let\TrackLangRequireDialect\noop@TrackLangRequireDialect
     \let\TrackLangAddToHook\@TrackLangAddToHook
     #1%
     \let\TrackLangRequireResource\noop@TrackLangRequireResource
     \let\TrackLangRequireResourceOrDo\noop@TrackLangRequireResourceOrDo
     \let\TrackLangRequestResource\noop@TrackLangRequestResource
     \let\TrackLangRequireDialect\@TrackLangRequireDialect
     \let\TrackLangAddToHook\noop@TrackLangAddToHook
   }%
   {%
     \@tracklang@warn{No `#2' support for dialect `#3'}%
   }%
}
\@tracklang@restore@at
\endinput
%%
%% End of file `tracklang.tex'.


==> vcm/cache-background.tex <==
\section{Cache Architecture}
ARM uses two bus architectures in its cached cores, the Von Neumann and the Harvard.
The Von Neumann and Harvard bus architectures differ in the separation of the instruction
and data paths between the core and memory. A different cache design is used to support
the two architectures.

In processor cores using the Von Neumann architecture, there is a single cache used
for instruction and data. This type of cache is known as a unified cache. A unified cache
memory contains both instruction and data values.

The Harvard architecture has separate instruction and data buses to improve overall
system performance, but supporting the two buses requires two caches. In processor cores
using the Harvard architecture, there are two caches: an instruction cache (I-cache) and
a data cache (D-cache). This type of cache is known as a split cache. In a split cache,
instructions are stored in the instruction cache and data values are stored in the data cache.
We introduce the basic architecture of caches by showing a unified cache in Figure~\ref{fig:caarch}.
The two main elements of a cache are the cache controller and the cache memory. The
cache memory is a dedicated memory array accessed in units called cache lines. The cache
controller uses different portions of the address issued by the processor during a memory
request to select parts of cache memory. We will present the architecture of the cache
memory first and then proceed to the details of the cache controller.

\begin{figure}
\center
\includegraphics[width=1\linewidth]{cacheDM.jpg}  
\caption{ A 4 KB cache consisting of 256 cache lines of four 32-bit words.}\label{fig:caarch}
\end{figure}

\subsection{BasicArchitecture of a Cache Memory}
A simple cache memory is shown on the right side of Figure~\ref{fig:caarch}. It has three main parts:
a directory store, a data section, and status information. All three parts of the cache memory
are present for each cache line.

The cache must know where the information stored in a cache line originates from in
main memory. It uses a directory store to hold the address identifying where the cache line
was copied from main memory. The directory entry is known as a cache-tag.
A cache memory must also store the data read from main memory. This information is
held in the data section.

The size of a cache is defined as the actual code or data the cache can store from main
memory. Not included in the cache size is the cache memory required to support cache-tags
or status bits.

There are also status bits in cache memory to maintain state information. Two common
status bits are the valid bit and dirty bit. A valid bit marks a cache line as active, meaning
it contains live data originally taken from main memory and is currently available to the
processor core on demand. A dirty bit defines whether or not a cache line contains data
that is different from the value it represents in main memory.

\subsection{BasicOperation of a Cache Controller}
The cache controller is hardware that copies code or data from main memory to cache
memory automatically. It performs this task automatically to conceal cache operation from
the software it supports. Thus, the same application software can run unaltered on systems
with and without a cache.

The cache controller intercepts read and write memory requests before passing them on
to the memory controller. It processes a request by dividing the address of the request into
three fields, the tag field, the set index field, and the data index field. The three bit fields are
shown in Figure~\ref{fig:caarch}.

First, the controller uses the set index portion of the address to locate the cache line
within the cache memory that might hold the requested code or data. This cache line
contains the cache-tag and status bits, which the controller uses to determine the actual
data stored there.

The controller then checks the valid bit to determine if the cache line is active, and
compares the cache-tag to the tag field of the requested address. If both the status check
and comparison succeed, it is a cache hit. If either the status check or comparison fails, ita cache miss.
On a cache miss, the controller copies an entire cache line from main memory to cache
memory and provides the requested code or data to the processor. The copying of a cache
line from main memory to cache memory is known as a cache line fill.

On a cache hit, the controller supplies the code or data directly from cache memory to
the processor. To do this it moves to the next step, which is to use the data index field of
the address request to select the actual code or data in the cache line and provide it to the
processor.


\subsection{Set Associativity}
Some caches include an additional design feature to reduce the frequency of thrashing. That is
a software battle for the same location in cache memory.
The result of thrashing is the repeated loading and eviction of a cache line.
This structural design feature is a change that divides the cache memory into
smaller equal units, called ways. Figure~\ref{fig:caarch-sa} is still a four KB cache; however, the set index
now addresses more than one cache line—it points to one cache line in each way. Instead
of one way of 256 lines, the cache has four ways of 64 lines. The four cache lines with the
same set index are said to be in the same set, which is the origin of the name ``set index.''

\begin{figure}
\center
\includegraphics[width=1\linewidth]{cacheSA.jpg}  
\caption{A 4 KB, four-way set associative cache. The cache has 256 total cache lines, which are
separated into four ways, each containing 64 cache lines. The cache line contains four
words.}\label{fig:caarch-sa}
\end{figure}

The set of cache lines pointed to by the set index are set associative. A data or code
block from main memory can be allocated to any of the four ways in a set without affecting
program behavior; in other words the storing of data in cache lines within a set does not
affect program execution. Two sequential blocks from main memory can be stored as cache
lines in the same way or two different ways. The important thing to note is that the data or
code blocks from a specific location in main memory can be stored in any cache line that
is a member of a set. The placement of values within a set is exclusive to prevent the same
code or data block from simultaneously occupying two cache lines in a set.



